ConfigTron: Tackling network diversity with heterogeneous configurations

The web serving protocol stack is constantly changing and evolving to tackle technological shifts in networking infrastructure and website complexity. As a result of this evolution, the web serving stack includes a plethora of protocols and configuration parameters that enable the web serving stack to address a variety of realistic network conditions. Yet, today, most content providers have adopted a "one-size-fits-all" approach to configuring the networking stack of their user facing web servers (or at best employ moderate tuning), despite the significant diversity in end-user networks and devices. In this paper, we revisit this problem and ask a more fundamental question: Are there benefits to tuning the network stack? If so, what system design choices and algorithmic ensembles are required to enable modern content provider to dynamically and flexibly tune their protocol stacks. We demonstrate through substantial empirical evidence that this "one-size-fits-all" approach results in sub-optimal performance and argue for a novel framework that extends existing CDN architectures to provide programmatic control over the configuration options of the CDN serving stack. We designed ConfigTron a data-driven framework that leverages data from all connections to identify their network characteristics and learn the optimal configuration parameters to improve end-user performance. ConfigTron uses contextual multi-arm bandit-based learning algorithm to find optimal configurations in minimal time, enabling a content providers to systematically explore heterogeneous configurations while improving end-user page load time by as much as 19% (upto 750ms) on median.

==> accuracy.tex <==

\subsection{Model Accuracy Analysis}
\label{s:benefits}
To analyze the accuracy of our models, we leveraged the simulator discussed in Section~\ref{}. Recall, in the large scale deployment, we have no ground truth and are thus unable to evaluate the acurracy and precisison of our models.  Here, we leverage the closed environment that the simulator provides to systematically analyze our algorithms.

\textbf{\BO Accuracy:}
\textbf{\RF Accuracy:}


Figure \ref{f:bestvsdefault-both} shows significant improvement in PLT when BO's recommended configuration is used over default configuration. However, we still don't know if this configuration performs equal to the best configuration possible or not. Finding the best configuration requires exploring the entire configuration space which is infeasible for a real-world deployment. To answer this, we leverage the data collected from our emulation test-bed and conducted experiments. For a certain network condition and website, 5 (init\_sample) samples are randomly selected and a BO model is trained. Once the optimization is completed (i-e thresholds are met), we compare PLT of BO recommended configuration with default configuration and best configuration available (found by exhaustive search through the configuration space). We run the simulation for 5 websites (ranging from content rich website like espn or amazon to simple webpage like google). For each website, we randomly select a network condition in each iteration and the simulations are run for 500 iterations.

Figure \ref{f:ei-emu} presents the results for simulation when a configuration space of size 142 was explored, keeping EI threshold as 5 and 10.
Figure \ref{f:ei-emu}(a,d) present the CDF for performance vs default configuration. For EI=5\% we can see improvement in PLT from 5-8\% for different websites in the median case, where as for 95th percentile the performance goes as high as 20-70\% for certain websites. 
msn.com seems to be the standout case, having performance boost as high as 70\% but at the same time requiring much more optimization steps to meet the thresholds, as compared to other websites. Looking at msn's PLT results, it shows a lot of variation in performance with changes in configuration, that leads to higher number of exploration (high EI due to variations) and hence a better working configuration.

Figure \ref{f:ei-emu}(b,e) present the CDF for PLT comparison when optimal configuration is compared with best configuration. Since BO is not guaranteed to find the best possible configuration, there are cases where best configuration has not been explored by BO and the thresholds are met. Tuning the threshold can allow BO to find the best configuration but requires much more optimization steps. As it can be seen, BO's recommended configuration delivers performance within 3\% of best configuration for 70\% of the cases, for 4 of the websites. Best configuration for espn works around 10\% than BO-recommended one.A look at BO's optimization steps for espn makes it clear that BO's expectation of improvement for espn is consistently lowest of the 5 websites, resulting in least number of steps in optimization and stopping at a configuration that is 10\% suboptimal than the best one.

\begin{figure}
	\centering
	\begin{subfigure}[b]{0.55\textwidth}
		\includegraphics[width=3in]{fig/combined-emu-142-5-full.png}
		\caption{EI = 5\%}
		\label{f:ei-5} 
	\end{subfigure}
	
	\begin{subfigure}[b]{0.55\textwidth}
		\includegraphics[width=3in]{fig/combined-emu-142-10-full.png}
		\caption{EI = 10\%}
		\label{f:ei-10}
	\end{subfigure}
	\caption{Effects of EI on optimization steps and optimality}
	\label{f:ei-emu}
\end{figure}

\begin{figure}[tbh!]
	\begin{center}
		\includegraphics[width=3in]{fig/init-samples.png}
		\caption{Number of optimization steps required.}
		\label{f:init-samples}
	\end{center}
\end{figure}


%\textbf{Time analysis:}
%To Do, different BO model for each hour of the day.

%\textbf{Comparison of SL vs ML:}

==> background.tex <==

	
\section{Background}
\label{s:bakground}

In this section, we presents a brief overview of the edge of CSP and CDN networks (Section~\ref{s:edgebackground}) and discuss source and implications of heterogeneity (Section~\ref{s:heterobackground}). 
% Next, in Section~\ref{s:motivation}, we demonstrate through controlled experiments that the benefits of configuration heterogeneity are substantial and parameter selection is non-trivial.

% and summarize by discussing challenges that impede edge support for heterogeneity (Section~\ref{s:challenges}).
\subsection{Edge of Online Server Providers}
\label{s:edgebackground}
We broadly define the edge of a CDN or CSP network as user-facing servers that end-users fetch content from.  For large CSPs, e.g., Facebook, the edges are located in collation sites and ISP PoPs (Point of Presense) around the world.  Smaller CSPs, e.g., CNN, pay CDNs, e.g. Fastly/Akamai, to use their servers as edge locations.

%Specifically, the content provider servers in points-of-presence (PoPs) (Figure~\ref{f:CSP:infrastructure}) for large providers, e.g. Google and Facebook~\cite{veeraraghavan2016kraken}, who own the data center and edge servers and content distribution networks (CDNs) for smaller providers that outsource their edge to CDNs, e.g., Akamai and Fastly~\cite{fastly:howcdnswork}, and maintain a set of origin servers in clusters.(Figure~\ref{f:CDN:infrastructure}). %


%https://docs.fastly.com/guides/basic-concepts/how-fastlys-cdn-service-works




%~\footnote{ we extend out definition to include proxies employed by either the ISP or the end-user because these proxies extend the edge of the content provider into the ISP's or end-user's networks}  
%In cellular and wireless networks, the configuration and placement of this edge significantly impacts performance over the last mile connection where latencies can be high.

The edge's web serving stack, Figure~\ref{f:networkstack}, consists of the TCP/IP protocol implementations, the web server (proxy) application, and content provider's web application (e.g., PHP or Java code). Traditionally, these edge servers employ broadly two different network stacks -- one for user facing connections and another for the data center facing connections. The data center facing connections are often optimized to fully utilize the backhaul links. Whereas the user facing connections are often fine-tuned to provide optimal performance in aggregate rather than to provide optimal performance per-client --- so they opt for improving the median across all users~\cite{dukkipati2010argument}. To account for differences between user devices, the edge often deploys special web applications that infer device type and adjusts the multimedia images, html, and javascript to optimize performance on the device. Essentially, the predominant approach is to reconfigure a service stack at Layer 7, e.g., upon detecting a mobile client, many content providers redirect users to a specialized mobile site.

%
% \begin{table*}[tbh!]
% 	\begin{center}
% 		%\begin{scriptsize}
% 			\begin{tabular}{|c|c|c|c|}
% 				\hline
% 				\textbf{Layer }&\textbf{Protocol Options} & \textbf{Config Granularity} & \textbf{Descriptions} \\ \hline
% 					{IP} & AS Peer & \\ \hline
% 				\multirow{9}{*}{TCP}&tcp\_congestion\_control & {Sock}, {S} &  \\ \cline{2-3}
% 				&initcwnd  (ICW)& {C} & \\ \cline{2-3}
% 				&tcp\_slow\_start\_after\_idle & {C} & \\ \cline{2-3}
% 				&tcp\_low\_latency & {C} & \\ \cline{2-3}
% 				&tcp\_pacing (sched\_fq) & {C} & \\ \cline{2-3}
% 				&tcp\_wmem & {C} & \\ \cline{2-3}
% 				&TSQ & {C}& Used to manage buffer bloat \\ \cline{2-3}
% 				&tcp\_autocorking & {Sock} &  \\ \hline
% 				{HTTP App} & HTTP Protocol & {C} &\\ \hline
% 			\end{tabular}
% 	%	\end{scriptsize}
% 	\end{center}
% 	%	\vspace{-0.2in}
% 	\caption{Web stack configurations parameters.}
% 	\label{t:configurations}
% \end{table*}


% \begin{table}[tbh!]
% 	\begin{center}
% 		CDN & InitCWND & TCP Version \\
%
% 	\begin{center}
% \begin{table}

%\begin{figure}[tbh!]
%	\begin{center}
%		\includegraphics[width=1in]{fig/NetworkStack.png}
%		%\vspace{-0.1in}
%		\caption{Network Stack.}
%		\label{f:networkstack}
%	\end{center}
%\end{figure}
%This papers explores the benefits of extending reconfiguration from the web application down to the server application and the TCP/IP stack -- and presents a system for realizing configuration in a principled manner.

%To deliver services with high performance, high reliability, and low latency for users, companies like Facebook, Google etc, use a multi-tiered networking infrastructure consisting of edge servers, points of presence (PoPs) and data center ~\cite{google}. Different levels of load balancing is being employed for high performance. DNS, layer-4 and layer-7 load balancing is used in case of data-centers to keep the performance level high by distributing the load on multiple back-ends. In case of CDNs and PoPs, DNS and layer-7 load balancing is used. The multi-tiered architecture presents a modular architecture, with an opportunity to introduce changes in front-ends for network stack reconfiguration, without any need to change the underlying infrastructure or users.
% ~\cite{https://peering.google.com/#/infrastructure} ~\cite{http://cs.unc.edu/xcms/wpfiles/50th-symp/Moorthy.pdf} 




 
%~cite{http://www.cisco.com/c/en/us/solutions/collateral/service-provider/visual-networking-index-vni/complete-white-paper-c11-481360.html}
%~\cite{https://www.akamai.com/us/en/our-thinking/state-of-the-internet-report/}


%Facebook:https://www.youtube.com/watch?v=H5jyM0oD418
%Google: https://peering.google.com/#/infrastructure



 \subsection{Heterogeneity in the Web}
\label{s:heterobackground}

 %In this paper, we are making a case for a "conditions-based configuration" strategy.
 
 \textbf{Heterogeneity at the congestion layer (TCP):} Although \textit{Cubic} is used as the default congestion control algorithm, the Linux kernel includes over 10 variants of TCP. Moreover various measurement studies show that different variants are optimal for different networking conditions ~\cite{song2006compound,floyd2003highspeed,hock2017experimental}. %For example, Compound TCP improves throughput in high-speed, long distance networks, and keeps its throughput lower-bounded by Reno~\cite{song2006compound} where HSTCP~\cite{floyd2003highspeed} was introduced by IETF as an experimental protocol that is suited for large congestion networks. 
 %Furthermore, others have shown that TCP performance can also be affected by routing protocols~\cite{tahiliani2013comparative,kim2006comparison}. 
 Orthogonally, others~\cite{dukkipati2010argument} have explored the impact of varying configuration parameters, e.g. initial window size on PLTs --- with the suggested default parameter evolving from 2 to 4 and now to 10 \cite{rfc6928}.
%
 In a largely counter-intuitive move, Google has adopted UDP over TCP in their design of QUIC~\cite{quic}, thereby introducing more diversity into the stack. 

 \textbf{Heterogeneity at the App layer (HTTP):} %HTTP/1.1 has been used for atleast the last decade. Google introduced 
 SPDY~\cite{spdy}, now HTTP/2, is now used uniformly by Google and others over HTTP/1.1. However, recent studies~\cite{wang2014speedy,erman2015towards} provide strong empirical evidence that HTTP/1.1 outperforms SPDY under certain network conditions (high loss rates and complex web-page dependencies).
 % and furthermore in a few situations SPDY performs worse than HTTP/1.1.

 \textbf{Heterogeneity at the End User:} Recent work~\cite{} has demonstrated that device characteristics impact the performance of different configuration options.  
% \textbf{Takeaway} While various measurement studies demonstrate the need for heterogeneous configurations, today's internet employs a "one size fits all strategy" where one set of configurations, suitable for a subset of the population, is used for the entirety of the internet.  We note that unlike these prior studies~\cite{dukkipati2010argument, ghobadi2012rethinking, wang2014speedy, erman2015towards} that explore a single protocol or configuration parameter, in Section~\ref{s:motivation} we present a more holistic exploration across multiple (arguably all) protocols and parameters.  Furthermore, unlike prior work~\cite{al2011overclocking} we present a concrete system (Section~\ref{s:archi}) to reconfigure and optimize the different protocols.
 
% \textbf{Takeaway:} Despite strong and growing evidence that optimal choice of configuration parameters are dependent on network conditions and web complexity, today most CDNs/CSPs employ homogeneous configurations.
% This papers explores the benefits of extending reconfiguration from the web application down to the server application and the TCP/IP stack -- and presents a system for realizing configuration in a principled manner.



 % \subsection{Challenges}
 % Listed below are some of the challenges in finding the optimal configrations for the web.
 %
 % \begin{itemize}
 % 	\item Non-deterministic nature of internet makes it harder for the performnace model to estimate the utility of a configuration.
 % 	\item Network conditions are subjected to changes and so does the performane of a configuration with it.
 % 	\item The relationship between performance model and network configurations is non-linear. Eg, keep increasing ICW would improve the performance to a limit and after that it can have adverse affects.
 % 	\item Not all the delays are network related. Server-related delays and complex website dependency graph makes it harder to estimate the performance.
   	
 %
 % \end{itemize}
 
 

==> critical_para.tex <==
\vspace{-0.15in}
\subsection{Critical parameters and features}
\label{s:critical-para}

Next, we analyze the relative importance of reconfiguring different configuration parameters. Our goal is to understand the crucial parameters that must be tuned to significantly improve performance. Figure~\ref{f:critical-para} plots the results for five configuration options. 
%\theo{how are these five selected?}

There are several crucial observations: while the HTTP parameter is crucial. It is not the most important and it is infact third after TCP-CC and ICW.
%
Unsuprisingly the congestion control algorithm (TCP CC) is the most important parameter because this directly controls throughput. The next important, ICW, is a related parameter that aids the congestion control algorithm.  
%
While there are many other parameters, e.g., Auto Corking, in the median case these provide little benefits but provide tremendous benefits at the tail. This implies that improving tail performance requires turning a broader range of parameters to account of the edge conditions that exist at the tail.
%The different configuration parameters may have different levels of impact on web performance and we are interested in finding how much performance gain tuning a certain parameter brings to the table. Another implication of this analysis is to reduce the configuration space eg, if all possible HTTP versions are delivering the same performance in a certain network condition, then there is no benefit to reconfiguring HTTP version and it can be excluded from the configuration space for the corresponding network condition. Let S be the set of all parameters. To decide if a parameter(P) is critical or not, we set rest of the parameters \{S - P\} to one of their possible values and evaluate performance by using different values for P.
% eg, to test if HTTP version is critical we test {HTTP=1.1, CC=cubic, ICW=4, AC=0, LL=0} and {HTTP=2, CC=cubic, ICW=4, AC=0, LL=0}. 
%If the performance differ by more than a user-defined threshold, the parameter is flagged as critical. Note that this comparison is repeated for every possible value of \{S - P\} parameters. Figure~\ref{f:critical-para} plots the results for five configuration options, averaged over all network conditions, using various thresholds (1\% to 100\%). 

% \begin{figure}[tb!]
% 	\begin{center}
%% 		\includegraphics[width=3.2in]{fig/critical_para_new.png}
%		\includegraphics[height=1.5in]{fig/para_threshold_v1.eps}
%		\vspace{-0.15in}
% 		\caption{Critical configuration parameters}
% 		\label{f:critical-para}
%		\vspace{-0.35in}
% 	\end{center}
% \end{figure}


% \begin{itemize} [topsep=0.1ex,leftmargin=0.5\labelsep]
% 	\setlength\itemsep{0em}
%
% 	\item TCP congestion control (CC) takes the first spot, with tuning just CC improving PLT as much as 15\% for the median case. The rationale behind this improvement is explained earlier in \ref{s:motivation}.
%
% 	\item TCP ICW comes next. A network-specific ICW helps in reaching the equilibrium faster \cite{tcpwise, dukkipati2010argument}, while at the same time doesn't overwhelm the network (\S \ref{s:icw-ten}).
%
% 	\item Tuning just HTTP results in significant improvements especially in high RTT, high loss networks, as well documented in \cite{wang2014speedy, erman2015towards}.
%
% 	\item TCP low latency improves performance in low latency environments.Sender advertises Maximum ACK Delay that improves loss recovery by computing a lower RTO. We observed this setting to be helping significantly in lossy networks. However, its effectiveness becomes negligible in no or low loss environments, rendering this setting non-critical in no or low loss.
%
% 	\item TCP auto corking allows the coalescing of small payloads to reduce the number of packets sent \cite{}. In our experiments, we found auto corking to be improving PLT by reducing the number of packets sent on wire.
%
% 	\item TCP pacing is found to be improving performance by reducing loss rate in low BDP (low BW, low RTT) networks.
%
%
% \end{itemize}


%We found Congestion Control to be the most critical, followed by ICW and then HTTP version. Tuning ICW results in atleast a 3\% improvement in PLT in 97\% of the cases. For Congestion Control and HTTP, atleast a 3\% improvement is observed in 91\% and 84\% cases respectively. TCP auto corking and low latency setting are much less than critical compared than their counter-parts, with the percentages dropping to below 50 for a 3\% improvement.





%In order to zoom into the affect of network conditions and criticality of a parameter, Figure~\ref{f:critical-para-tree} presents a decision tree. The tree is built using a threshold of 1.5\%. The leaves represent percentage ranges for the total number of cases when a parameter is critical. 
%Congestion control lowest criticality values ($\sim$70\%) are seen at high RTTs (\textgreater  250ms) and bandwidths \textgreater  5.5Mbps -- meaning tuning congestion control is critical 70\% of times in these network conditions. Auto corking and low latency seems to follow an identical pattern and become highly critical ($\sim$85-90\%) when RTTs \textless  48ms. HTTP and ICW criticality stays high ($\sim$85\% and higher) in all network conditions.
% \begin{figure*}[tbh!]
%	\begin{center}
%		\includegraphics[width=6.5in]{fig/critical_para_tree.png}
%		\caption{Critical configuration parameter's relation with network conditions}
%		\label{f:critical-para-tree}
%	\end{center}
%\end{figure*}


==> design_challenges.tex <==
\section{Design Challenges and Future Works}
\label{s:discussion}
Our design and prototype explore a single point in the design space. In this section, we discuss alternate design points and their implications.

\textbf{Learning Network Conditions:}
Our current design infers the client's network conditions based on packets exchanged between servers and the clients; in a similar fashion to how TCP learns a client's network conditions. An alternate and more direct approach is to have the clients explicitly probe, capture and exchange network condition information with the servers. This can be done by modifying the client software stack~\cite{yiakoumis2016neutral} to actively probe the webserver or adding javascript or invisible images into the webpage that enables the webserver to collect client-side statistics~\cite{ghasemi2016performance}. As part of future work, we plan to explore the more accepted approach: embedding javascript or images for performance profiling.



%
% \subsection{Data collection for learning}
% One of the most important part of the system design is the \textit{Learning Module} (LM). LM is responsible for finding the most optimal TCP stack configuration for a given client, according to her network conditions. As a start it will use the data about best configurations found from the experimentation and will further build on it by learning online from the clients served. An important question is: \textit{How will LM get the information about network conditions from clients?}. This information exchange can happen in two ways:
%
% \textbf{Implicit learning:} LM will learn about user's network conditions (bandwidth, loss rates, RTT) implicitly i-e there would not be an agent running on client. In this case clients would need no modification. For implicit learning, TCP dumps at the servers can be used.
%
% \textbf{Explicit learning:} There will be agents running on clients that will actively exchange information with LM. In this case, clients will need to be modified.
%
% There are pros and cons of both techniques. Implicit learning has the advantage of no client modification but explicit learning has the advantage of being more accurate than implicit one.



% \subsection{Granularity of learning}
% Another important aspect of learning is to decide the granularity of learning. There can be multiple levels for learning.
%
% \textbf{Prefix based:} \textit{Learning Module} will learn about network conditions for clients belonging to a certain IP prefix. For the entire set of users for the prefix, \textit{Learning Module} will recommend a single TCP stack configuration. A single configuration will be used for a set of users.
%
% \textbf{IP based:} Learning will be a granularity of each, individual client. For each user, \textit{Learning Module} will recommend a single TCP stack configuration.
%
% % IS THAT RIGHT?
% \textbf{Connection based:} At the beginning of each connection, \textit{Learning Module} will recommend the most-optimal configuration. There will be no need for maintaining history for the clients.
%
% Each level presents a trade-off between storage complexity and performance faced by clients. If prefix are used, less storage space is required for matching clients to configuration but the configuration might not be the most optimal for each client. In case of IPs, each the optimal configuration will be used for each client but keeping record of large number of IPs and their configuration can be an issue. Connection based approach will suffer from the over-head of finding the optimal configuration at the beginning of each connection.




%
% Let's assume that the \textit{Learning Module} is actively learning about the client conditions at each request/response. Since client's network conditions (bandwidth, loss rates, RTT) can change at any moment in time, \textit{Learning Module} can recommend some different configurations for the same client at some future point. A question arises: \textit{How often should the system reconfigure the TCP stack for a client?}. There can be three cases:
%
% \textbf{Every packet} If LM recommends a different configurations for the client, the stack needs to be reconfigured before sending the next packet. In other words, the next packet will be sent using the new configurations. In this case, every packet will be sent with the best configuration, as recommended by LM.
%
% \textbf{Every object} If LM recommends a different configurations for the client, the stack needs to be reconfigured before sending the next object. In this case, if the LM's recommended configuration changes, the system will wait for the current sending object to be sent with the previous configurations and then reconfigure.
%
% \textbf{Every connection} In this case, the stack will be reconfigured the next time client makes a connection with system. So learning will be used for making the future connections better.







% \subsection{Not a traditional load balancer}
% The \textit{Request Router} is not a traditional reverse proxy or a load balancer in the sense that it is not involved in the response. I traditional proxy or load balancer forwards the request to back-end, gets the response from back-end and forwards the response back to client. Whereas our \textit{Request Router} is only involved in forwarding the request part. The reason being, if \textit{Request Router} is used in forwarding the request back to client, its TCP stack configuration will be used in sending the request back to client whereas we need to ationuse the VM's TCP stack configuration for the response.
% Another approach that can be used is to use DNS-based load balancing. DNS load balancer will take place of \textit{Request Router}. When client makes the DNS query for front-end's IP address, the IP of the corresponding VM will be returned as the response of DNS request. \textit{Time to live (TTL)} for DNS records needs to be small so that if the \textit{Learning Module} recommends some new configuration (and a different VM as a consequence), the client does not keep using the old, stale DNS entry of previous VM.
%
% \subsection{Layer-3 forwarding}
% \textit{Request Router} needs to be operated at layer-3 level and should forward the request based on client's IP. This is required for since the TCP handshake needs to between client and VM. Otherwise the client will not be able to match responses from the VM to the requests sent. Let us consider the case of using forwarding based on layer-7. Client will setup TCP connection with \textit{Request Router} and will get no response from \textit{Request Router}. The request will be forwarded to VM, which will then send the response back to client. Since the client's original TCP connection was with the \textit{Request Router}, it will not  be able to match response to request (the remote IPs and TCP sequence numbers in request/response will not match).





\textbf{Configuration Granularity:}
Our current design reconfigures the webstack at the granularity of a VM --- with each VM containing a distinct set of configuration parameters.  While heavy weight,  VM-level configurations allows us to reuse existing and mature tools while providing full control over all configuration parameters.  Alternatively, we could explore containers (e.g. LXC or Docker) as the granularity of control. However, since containers share the same network stack, we would need to use space TCP/IP protocols to provide control over certain TCP configurations, e.g., TCP version. As part of future work, we plan to explore a fusion of both extremes.  Namely, leverage VM-level granularity for controlling kernel-level global parameters, e.g., TCP version, and container-level granularity for controlling connection-level local parameters, e.g., HTTP protocol version.


\textbf{Reconfiguration Frequency:}
Our current design reconfigures the web stack at the beginning of each connection. This limits the flexibly of \sysname and prevents us from adapting to drastic changes in the end-user's networking conditions. Alternatively, we could reconfigure the stack at finer granularities, i.e., before every packet or before every object.  Although reconfiguration at the finer granularity enables us to react more finely, and ultimately to improve performance, finer granularity introduces several significant challenges, e.g., managing reconfiguration overheads and tackling the implications of reconfiguration on existing state for the connection.


\textbf{Reconfiguration Overheads:}
There are some over-heads associated with reconfiguring the web stack, specifically, VM setup cost (e.g. image transfer and bootup) and kernel reconfiguration (e.g. changing the protocol version). To tackle these overheads, we plan to explore a combination of approaches to ameliorate this overheads, e.g., maintaining a fleet of preconfigured VMs and proactively scale-up this fleet in respond to fluctuations in demand.

%Due to the presence of these over-heads, selecting the granularity of reconfiguration becomes a question of finding the right balance between reconfiguration over-heads and performance gain from using reconfigured stack. In case of "every packet reconfiguration" the associated over-heads will be highest (since the system might need reconfiguration after sending every packet) but the performance gain will be highest (since each packet will be sent with the most optimal configuration). Moving from "every packet" to "every connection", reconfigurations over-heads decreases but the performance gain will be lower than the "every packet" case. 



% since the kernel will take in some amount of time to plug-in the new TCP congestion protocol or update new \textit{initcwnd} values in IP tables. Note that, instead of reconfiguring a VM, if a VM with the required configuration in already present, we can just reroute the next requests to that VM. This would lower down the reconfiguring over-heads but there would be need for session migration to the other VM.



\textbf{Deployment Scenario:}
The current design explores a point in the design space that requires content-providers to modify and improve their infrastructure. Yet, there are also points in the design space; 
%
% \begin{itemize}
% \item the first, 
where the content-provider and the end-user cooperate, these points in the design space enable us to explore a broader range of configuration options including configuration on the end-user client and explicitly exchange of client side information.  Although this approach appears altruistic, this point in the design space can be easily explored by large online service providers, e.g., Facebook and Google. As part of future work, we plan to explore the additional benefits that arise from leveraging client (end-user) cooperation.

% \item the second, where the content-provider is not involved and the end-user leverages a proxy, in the cloud, to split connections, reconfigure parameters, and improve QoE metrics. Unfortunately, this approach requires clients to place trust in the proxy and manipulate SSL to incorporate the proxy. We plan to explore the use of recent extensions to TLS to explicitly include middleboxes.  Given this stronger trust model, the proxy can incorporate more sensitive information from the client to enable more aggressive configuration such as selective compression, HTTP-2 push, and HTTP-2 priorities.
%
% %Similar, to the use of split TCP-proxies to improve performance over wireless, we expect that this approach will
%
% \end{itemize}

% The deployment depends on the level of cooperation between the different entities. We focus on the more realistic scenarios, where a user or a content provider unilaterally decides to employ \name. We ignore the scenario where in the ISP unilaterally decides to employ because the widespread use of TLS prevents the ISP for covertly(transparently) employing a proxy.
%
% \textbf{End-User} When the end user employs \name, the end user will need to for all traffic to go through \name's proxy service. We envision that the end-user will deploy the proxy as a light weight process within the cloud, e.g. PicoCenter~\cite{}, and employ ssl-XXX to allow the proxy to interpose on encrypted traffic. The user can have a local agent running for exchanging information with the proxy. However, this is not the only way and implicit information exchange is also possible. We are going to further discuss this in next section.
%
% \textbf{Content-Provider} This provides with a more interesting situations as the content provider must infer information using existing fingerprint techniques and existing active and passive probing techniques.  Given this information, the content provider can run \name on its edge servers. Thus allowing the edge servers to adjust to specialize to an end user's local conditions.
%
% We are going to focus on edge of CDN as a candidate for \name deployment as the CDNs already store data about clients for personalization. Edge of a CDN is also a better candidate for \name deployment since this will preserve the multi-server nature of websites. Let us consider \name as a black-box that uses a personalized TCP stack for each user. Figure~\ref{f:proxy_vs_cdn} shows how this black-box will be used for forwarding requests.
%
% \begin{figure}
% 	\begin{center}
% 		\includegraphics[width=3in]{fig/proxy_vs_cdn.jpg}
% 		\caption{Different deployment scenarios}
% 		\label{f:proxy_vs_cdn}
% 	\end{center}
% \end{figure}

%
% % NEED TO DISCUSS
% \subsection{Learnign algorithm}
% Simple decision tree based model or clustering.
% To be added.  Need to discuss.
%
% % NEED TO DISCUSS
% \subsection{Stack flexibility}
% — L7 (HTTP app), L5 (TLS ), L4 (TCP), L3 (IP)
% To be added. Need to discuss.

 

%
% Although instead of VMs, it would have been more efficient to use containers (like LXC and Docker) with reconfigured TCP stacks, they do not provide the level of isolation that we needed. Eg, containers running on a host machine shares hosts's \textit{tcp\_congestion\_control}. However, the number of VMs required can be minimized by using containers with VMs. Let us consider the case of \textit{TCP congestion protocol}, \textit{initcwnd} and \textit{HTTP version}. A single VM will use a single \textit{TCP congestion protocol} but can support multiple \textit{initcwnd} and \textit{HTTP version} with the help of container. Eg, {cubic, initcwnd=4, http/1.1} and {cubic, initcwnd=12, http/2} can be supported by the same VM having cubic as \textit{TCP congestion protocol} and two containers, one with initcwnd=4 and using http/1.1, other with initcwnd=12 and using http/2.
%
%
% \subsection{User-space TCP/IP stacks:}
% Another approach that can be used in place of VMs is to use user-space TCP/IP stacks inside containers. We tested with \textit{Light Weight IP (lwIP)} ~\cite{dunkels2004lwip} and \textit{mTCP} ~\cite{jeong2014mtcp} and found their TCP stacks to be lacking in features. Eg, no vegas support.


==> end-to-end.tex <==
\subsection{End-to-end evaluation}
\label{s:latency}

\obj{(i) NC classification should be on (user,CDN server) pair level. For a big CDN, a single client may classify into different classes for different CDN servers, eg, client C to CDN server 1 latency is 20ms, C to CDN server 2 latency is 50ms. Then it might be sorted into different NCs. (ii) What will be the number of NCs in a real setting? It will be some sort of combination on number of network conditions, device types etc.}

\subsubsection{Impact of latency}
\obj{how does latency between learnign agent and config manager/agent impact the performance?}

\obj{Ran a new experiemnt here. This one was for a subset of trace and only focuses at the start of learnign. Things should be pretty different at later stages. }

In a real-world setting, there might be some latency in updating rules at \textit{Config. Agent} by \textit{Learning Agent} due to the physical distance between the two actors. Figure \ref{f:end-to-end-latency} shows how improvement in PLT suffers as latency increases. However, the takeaway observation is that most of the sub-optimality due to higher latencies is limited to the start of learning process. After some time has passed and the learning model has matured, the sub-optimality, due to latency in updating rules at learning agent, decreases.

\begin{figure}[tb!]
	\begin{center}
		\includegraphics[width=3in]{fig/end-to-end-latency-f-v1.eps}
		\caption{Impact of latency}
		\label{f:end-to-end-latency}
		\vspace{-0.2in}
	\end{center}
\end{figure}




==> learningspeed.tex <==
\subsection{Learning speed}
\label{s:learning}
\sysname learning function is required to reach the optimal configuration quickly, as any A/B tests can adversely affect end-user's QoE. For SL learning speed is defined as the number of optimization steps needed to meet thresholds. Whereas, for ML learning speed is attributed to the amount of data required to a certain accuracy score.

\textbf{SL:} Number of optimization steps is controlled by EI and min\_sample\_tested thresholds. Once we have enough number of initial samples (init\_sample=5) for a network cluster, a BO model is built. In each optimization step, BO recommends the next configuration to be tested and the performance result from the actual test is fed back to BO model. Once we have reached enough number of test samples (min\_sample\_tested=8) and EI for the next recommended configuration gets lower than threshold (10\%), optimization is stopped.
Figure \ref{f:opt-step} presents the number of optimization steps needed to reach the thresholds. For the median case, EI threshold was reached within 3 optimization steps. For 85\% of the cases, BO stops within 5 optimization steps while for 99\% of all the cases, BO meets the thresholds after exploring half or less than half of the configuration space.

Steps < 3 seems improbable since atleast three optimization are required to reach the threshold min\_sample\_tested=8  from init\_sample=5. However, for CDF shows that for around 25\%, less than 3 steps are required. This happens when network conditions of a client changes midway connection. BO assigns a different network cluster to the client, but the client's ongoing connection keeps using the previous configuration until its done. BO also include their different configuration and its performance into optimization step and as a result more than one configurations are sampled in a single optimization step. This allows for reaching min\_sample\_tested in less than 3 steps.

\begin{figure}[tbh!]
	\begin{center}
		\includegraphics[width=3in]{fig/opt-step-cdf.png}
		\caption{Number of optimization steps required to reach thresholds}
		\label{f:opt-step}
	\end{center}
\end{figure} 
%TO further explore the BO's learning speed, we leverage our emulation test-bed. 

\textbf{ML:} We use the data from deployment to find the right amount to data to need a certain accuracy thresholds. We divide the data into training (90\% of all data) and testing (10\% of all data) samples. Starting from, scratch in each iteration we train the model on a batch of 10 data points from training set and cross-validate it using testing set. Figure \ref{f:data-acc} plots accuracy vs amount of data required to reach certain accuracy. About 20\% of the training data is enough to cross 90\% accuracy.

\begin{figure}[tbh!]
	\begin{center}
		\includegraphics[width=3in]{fig/data-vs-acc.png}
		\caption{Amount of data required to reach a threshold}
		\label{f:data-acc}
	\end{center}
\end{figure} 


==> naive.tex <==
\section{Strawman Approach}



\subsection{Design Goals}\label{s:designgoals}

We can summarize our observations as follows: configuration heterogeneity is beneficial for improving the performance of different clients; while different clients require different configuration parameters, most clients can achieve close to optimal by exploring a limited set of ``golden'' parameters; and, the choice of parameters are predicated on features of the clients network and website.  Based on these observations, we identify the following design goals for enabling edge servers with heterogenous configurations.
\begin{itemize}
\item \textbf{Accurate and fast learning} Using a limited number of observed data points about network conditions and their optimal configurations, \sysname should be able to predict the optimal configuration with high accuracy. It should also be able to infer if the observed data points are not enough.

\item \textbf{Isolation:} Different clients require different configuration as such the scope of a set of configuration parameters should be limited to the
 intended connection(s). Further, the costs and overheads of reconfiguring the web server to support these parameters should
  be limited to the connection. For example, changing the TCP protocol should not require an application restart (or worse a server restart).
  %Failure or recovery of one \SDNapp should not affect the other (healthy)
  %\SDNapps. 
  %Isolation of \SDNapps promotes high availability and simplifies
  %failure recovery.
  % efforts.

  
\item \textbf{Minimal Operator Effort:} While manual reconfiguration is the source of most outages~\cite{}, today, operators remain involved in fine-tuning the web stack. We argue that for the edge to successfully support fine-grained heterogeneous configuration (and reconfiguration), the process must be fully automated.  


\item \textbf{Minimal Management Overhead:} While automation improves efficiency and reduces outages, automation can complicate management and debugging.  Specifically, when operators are trying to diagnose operational issues, many tools need to know the exact configuration and potentially group based on these configurations -- a first step towards reducing the debugging complexity will be to minimize the number of optimal configurations deployed in production (N).


\item \textbf{Fast Reconfiguration:} Web performance is highly impactful, with studies~\cite{} showing that an additional 100ms increase in PLT can result in a significant loss in revenue.  Thus, reconfiguration should happen in a timely manner. More broadly supporting heterogeneity should not significantly impact a client's page load times.


\item \textbf{Scalable:} Edge web servers are kept minimal to support scalability and high performance. Introduction of heterogeneity should not compromise scalability of the existing system.
  %further inducing failures and crashing the \SDNapps.
  
%\item Management Overheads: There are some management over-heads associated like like storing optimal configuration for billions of users. A simple IP based approach will lead to storage and lookup over-heads.




\end{itemize}

==> network-change-point.tex <==
\subsubsection{Detecting change in network} 
\label{s:network-change-point}

Due to changing network conditions, \sysname's expectation of a user's network class may diverge from the ground-truth. As a result, any prediction made on the basis of this stale expectation might be sub-optimal.
\sysname uses observations from \cite{imc:hobbit} to monitor homogeneous blocks of IPs and generalize any change in network for one IP to its whole homogeneous block. As a result, sub-optimal predictions due to changes in network is limited to just first user of homogeneous block for which network change was first observed and the change in network is propagated to the rest of the block. Recent works \cite{sigcomm:cs2p} leverage piece-wise stationary nature of long-lived TCP connections to predict any change is state. However, we didn't pursue this direction of adding complex Hidden Markov or LSTM models due to comparatively short-lived nature of TCP connections for most of web, in contrast with video streaming. 
%As the network stays stable in oder of seconds to minutes,   

\usama{This part needs changes or perhaps removing the hobbit part as its not helping much in actual.}

==> new-evaluation.tex <==
\section{Evaluation}
Our evaluation of \sysname is motivated by the following questions:
%
 What are the empirical benefits of using \sysname? (Section~\ref{s:benefits})
 %
%Which operating conditions are the different learning algorithms better fit for? (Section~\ref{s:comparison})
 %
How sensitive are the different learning algorithm to the hyper parameters? (Section~\ref{s:sensitivity})
%
What are the overheads of \sysname on the web servers? (Section~\ref{s:overheads})

\subsection{Experiment Setup}

To understand and quantify the benefits of reconfiguring the networking stack, we conduct a large scale study to determine the optimal configurations for the different network conditions. 

We evaluated \sysname using both a live deployment and a network simulation. Together, these two experiments allow us to understand the behavior of \sysname under real and dynamic conditions as well as to simultaneously analyze the implications of individual design choices on the entire systems.

\parab{Live Deployment} We deployed \sysname on three servers with 12 cores Intel(R) Xeon(R) CPU E5-2620 @ 2.00GHz and 16 GB of RAM. In this deployment, one server runs \sysname-enhanced web server and the other runs the web server with vanilla configurations and the last server is used to host the \manager. 

For our live deployment, we developed a web client in 105 LoC in python using Selenium and PhantomJS. These web clients periodically to conduct back-to-back requests for a \sysname-version of the website and a vanilla version of the website. We deployed this client software on a combination of PlanetLab nodes and Bismark routers. 
\theo{PlanetLab clients are linux machines, using Fedora 8 distribution. BISmark's insfrastructure includes a variety of device, ranging from Raspberry Pi to routers used in home networks. Each configuration and website is tested multiple times, to minimize the effects of variations in internet.} In total, we had approximately 100 clients each configured to load 10 websites every 15 minutes. This provided us with more than 600,000 data points over a 7 day period.

\theo{we need to discuss difference between synthetic and real pages. also impact of network. we also need to add more parameters.}


\parab{Large Scale Simulations:} With our live deployment, we are unable to collect the ground truth, i.e., the optimal configuration, because this requires a brute-force search through the configuration space.  To better understand the accuracy and the upper bounds of \sysname relative to the optimal, we developed a large scale simulator that focuses on the interactions between the \manager and the clients.

Our test-bed comprises of a cluster of 300 servers. Our servers used Linux kernel 4.9 (BBR became available as a plug-able congestion control mechanism from 4.9 to onwards). The servers are configured to use both HTTP versions, multiple congestion control including BBR and other configuration options listed in Table~\ref{t:configurations}. We use chromium \cite{chromium} as the client and the process is automated using Selenium and Python. We used NetEm \cite{netem} and TC \cite{tc} for emulating network between clients and servers and test a range of websites (both synthetic and real-world web pages).

We collected packet traces for real-world sessions to simulate page loads in our test bed. The packet traces come from three different sources: FCC~\cite{fcc}, CAIDA~\cite{caida} and MAWI~\cite{mawi}. We looked at a cummulative $\sim$(6 + XX)M sessions (FCC 1.6M, CAIDA 4.5M, MAWI XXM)
The three data sources provide a good coverage over a wide range of representative network conditions and diverse clients. We sift through the packet traces to measure network conditions faced by the end-users. We model each end-user as a time series -- measured network conditions indexed over time. The time series enable us to simulate client sessions by modeling the changes in network conditions faced by the clients. We cluster the network conditions seen in time series to find the set of representative network conditions. Taking this test-bed as the input, a brute force and exhaustive search is performed across combinations of configuration, network, and website combinations creating a large tensor.

Given this large tensor, we are able to simulate clients with different network behaviors and observe both (1) which configuration \manager will assign to these clients and (2) the performances that these clients will receive. Our simulator reuses the code for \manager and merely simulates the client and webserver interactions.

\textbf{Limitations:}
%The test-bed loads a page a single time in a single session. 
The test-bed isn't able to evaluate configuration like tcp\_slow\_start\_after\_idle that affect TCP flow when a client re-engages with the server at a later stage in the same session. Similarly, the testbed isn't able to evaluate HTTP configurations parameters max concurrent streams and max number of connections as their affects only become visible under heavy load.






==> observed-vs-optimal.tex <==
\subsubsection{Observed vs Optimal}
\label{s:obs-vs-opt}

Here, we compare the performance implications of the configurations fingerprinted in Table \ref{t:ig} with \sysname-predicted configurations for a variety of websites, under 30 realistic network conditions observed in real-world traces.


 \begin{figure}[tbh!]
	\begin{center}
		\includegraphics[width=3.2in]{fig/plt_emu_results_bar.eps}
		\caption{Benefits of using Configtron for real cases}
		\label{f:obs-vs-opt}
	\end{center}
\end{figure}

==> offline-learning.tex <==
\textbf{\sysname's learning algorithm outperforms offline models, leveraging A/B testing.}
\label{s:offline-learning}
Network conditions can be radically different in different regions. We modified the simulator to replace online, A/B-testing based learning with an offline-model, built using data from simulator. Figure \ref{f:offline-learning} plots the results when the offline model uses network conditions from Japan and test it for traces from US. The first two box-plots show improvement for different data sets, while the third shows the actual improvement  observed by using \sysname.

As it can be seen, the observed improvement in PLT takes a hit, owing to the different network conditions in training (Japan) and testing (US) traces. An effective offline model will need to cover the entire spectrum of different networking conditions.

\begin{figure}
	\begin{center}
		\includegraphics[width=1.5in]{fig/data_locality.eps}
		\caption{Impact of data locality}
		\label{f:data-locality}
	\end{center}
\end{figure}

\textbf{\sysname's learning algorithm is not sensitive to data locality.}
Building on the offline version of \sysname, we introduced online learning and A/B testing to the offline model to observe the impact of locality of data. Any NC present in offline model is already mature and does not need further exploration. Figure~\ref{f:data-locality} plots the results when it is compared with regular \sysname. The offline model is based on traces from Japan and is evaluated for traces from US. We do not observe any significant impact of data locality. An eye-ball analysis of the network conditions of the two traces showed that there's little overlap between the two's NCs, with traces from Japan having 47\% lower number of NCs. More importantly, only 17\% of NC overlap between the two, thus limiting the benefits of using offline model.





==> old_eval.tex <==




%\subsubsection{\sysname ML:} 
%In the ML version, we use Random Forest as the learning function to predict the future configurations. The process of building random forests is described in Section \ref{s:learning}. It has been already established by the empirical evidence presented in Section \ref{s:motivation} that reconfiguring network stack leads to improvement in performance. In the evaluation of \sysname ML, we are concerned with the evaluating the improvement in performance and accuracy of prediction by \sysname's learning function.

%For evaluation, we tested the \sysname ML prototype for more than a weak with realistic clients. By going through the hyper-parameter space, we found the set of random forest tuning parameters that served us the best. We used entropy for the information gain as the measure of quality of split, 64 number of trees in the random forest and sqrt(number of features) as the maximum number of features. We did not limit the depth of the trees and used 2 as the minimum number of samples required to split a node. 

%For training the random forest, the prototype juggles through the configuration space to evaluate the performance of different network configurations in diverse network conditions. Figure \ref{f:bestvsdefault-both} presents the CDF of improvement in PLT when optimal configuration, predicted by random forest, is used instead of default configuration. In the median case, we can see an 7\% improvement in PLT. For the 95th percentile, we can see an improvement of more than 25\%. For around 9\% of scenarios, we can see a negative improvement in the PLT, corresponding to the cases when the configuration used for a client is sub-optimal as compared to the default configuration. This happens in the active learning phase, when a newly selected configuration in A/B tests is used for a client to bootstrap the learning process and gather training data. Since we don't know about the expected performance of a configuration before actually testing it, it can perform sub-optimally than the default configuration. As time progresses, the ML model incrementally trains on A/B tests performance results and is able to predict the favorable configuration for a user. 
%Zooming into the regions where we experience highest improvements, we find that this improvement is attributed to high value (25-30) being used. The bandwidths in these regions lie between 300-500Kbps with RRTs ranging from 35-45ms and minimal packet loss rates (0-0.1\%). Majority of the websites exhibiting greater than 20\% improvement are content-rich, eg sports, news etc. As it can be seen from the CDF, the region with 0\% improvement is minuscule, indicating that there's only a very few number of cases when random forest recommend using the default configuration. (0\% improvement is for the case when default and favorable configuration are the same).


%Random forest can internally calculate the error and accuracy of the model by calculating out-of-the-bag(OOB) score. In a random forest, each tree is initially bootstrapped with random data samples. If S is the entire dataset and S\textsubscript{k} represents data used for bootstrapping kth tree, then OOB score is calculated by using \textit{S - S\textsubscript{k}} data for the kth tree. \sysname's random forest based learning function  was able to get an OOB score of \textbf{96.2\%}. We also calculated the accuracy of our model by cross-validation and found our model to be \textbf{96.3\%} accurate in finding the optimal configuration. Since \sysname uses A/B tests for exploring new network conditions (section \ref{s:learning}), more data points are fed to the model with the passage of time and the accuracy is bound to be improved. Figure \ref{f:conf-mat} shows the confusion matrix of random forest, and as it can be seen from the diagonal values, the model predicts the correct configuration with extremely low false positives and the classes are balanced.

%\begin{figure}
%	\begin{center}
%		\includegraphics[width=3.2in]{fig/default_vs_best_ml.png}
%		\caption{CDF of PLTs for Default vs optimal config -- ML case.}
%		\label{f:bestvsdefault-ml}
%	\end{center}
%\end{figure}

%\textbf{Training data size and model accuracy:}




%\subsubsection{\sysname SL:}
%We tested \sysname SL deployment against realistic end-users for a week. Our prototype requires three inputs from the user: (i) number of initial samples for the Bayesian optimization model, (ii) threshold on minimum number of samples and (iii) expected improvement (EI) threshold. We tested a multitude of these parameters and found init\_sample=5, min\_sample\_tested=8 and EI=5\% to be the most suitable. Note that, EI controls the trade-off between exploration and accuracy. Smaller EI values may lead to better configurations but will require more exploration time. 


%We are interested in four aspects: (i) Improvement in PLT for optimal over default configuration, (ii) How long does it take to reach the optimal configuration, (iii) For similar network clusters, does the optimal configurations change over time, and (iv) The affect of threshold parameter on final outcome.

%For these measurements, each experiment was performed for a time interval of T hours, that is after T hours a new BO model was generated from scratch. We used this strategy to test if similar optimal configurations are generated in different runs and if the results from one run can be generalized to another. 

%For the experiments, we set T=3 hours.

%\textbf{Improvement in PLT:}
%Figure \ref{f:bestvsdefault-both} presents PLT comparison when optimal configuration (found by BO-based learning function) is used versus default configuration. For the median case, we measured around 12\% improvement in PLT. For the 95th percentile, PLT was reduced by as much as 50\%.

%\begin{figure}[tbh!]
%	\begin{center}
%		\includegraphics[width=3in]{fig/plt-cdf-sl.png}
%		\caption{CDF of PLTs for Default vs optimal config -- SL case.}
%		\label{f:bestvsdefault-sl}
%	\end{center}
%\end{figure}

%\textbf{Time to reach optimal configuration}
%\sysname learning function is required to reach the optimal configuration quickly, as any A/B tests can adversely affect end-user's QoE. Time to reach the optimal configuration is controlled by EI and min\_sample\_tested thresholds. Once we have enough number of initial samples (init\_sample=5) for a network cluster, a BO model is built. In each optimization step, BO recommends the next configuration to be tested and the performance result from the actual test is fed back to BO model. Once we have reached enough number of test samples (min\_sample\_tested=8) and EI for the next recommended configuration gets lower than threshold (5\%), optimization is stopped. Note that optimization steps will carry on until both of the thresholds are met.
%Figure \ref{f:opt-step} presents the number of optimization steps needed to reach the thresholds. For the median case, EI threshold was reached within 4 optimization steps, with the number of samples tested being greater than min\_sample\_tested (8). Note that, time T can also limit the search for optimal configuration. In these experiments we set a limit on maximum number of optimization steps to be 25. For 12\% of cases the two thresholds were not met within 25 optimization steps. However, the improvement over default configuration was still significant, even when the thresholds were not met (19\% PLT improvement on average). Increasing the EI threshold to 8\% allows 100\% of experiments to reach thresholds with 25 optimization steps, with significant PLT improvement (8\% for median case). 
%
%\begin{figure}[tbh!]
%	\begin{center}
%		\includegraphics[width=3in]{fig/opt-step-cdf-sl.png}
%		\caption{Number of optimization steps required to reach thresholds}
%		\label{f:opt-step}
%	\end{center}
%\end{figure} 

%\textbf{BO emulation experiments:}
%Figure \ref{f:bestvsdefault-both} shows significant improvement in PLT when BO's recommended configuration is used over default configuration. However, we still don't know if this configuration performs equal to the best configuration possible or not. Finding the best configuration requires exploring the entire configuration space. To answer this, we leverage the data collected from our test-bed described in Section \ref{s:motivation} and conducted emulation experiments. For a certain network condition and website, 5 (init\_sample) samples are randomly selected and a BO model is trained. Once the optimization is completed (i-e thresholds are met), we compare PLT of BO recommended configuration with default configuration and best configuration available (found by exhaustive search through the configuration space). We run the emulation for 5 websites (ranging from content rich website like espn or amazon to simple webpage like google). For each website, we randomly select a network condition in each iteration and the emulations are run 500 iterations.
%
%%\begin{figure}[tbh!]
%%	\begin{center}
%%		\includegraphics[width=3in]{fig/combined-emu-36-5.png}
%%		\caption{Emultaion results for 36 configurations and EI=5\%}
%%		\label{f:combined-emu-36-5}
%%	\end{center}
%%\end{figure}
%
%Figure \ref{f:ei-emu} presents the results for emulation when a configuration space of size 142 was explored, keeping EI threshold as 5 and 10.
%Figure \ref{f:ei-emu}(a,d) present the CDF for PLT comparison when optimal configuration is compared with default configuration. For EI=5\% we can see improvement in PLT from 5-8\% for different websites in the median case, where as for 95th percentile the performance boost goes as high as 70\% for certain websites. msn.com seems to be the standout case, having performance boost as high as 70\% but at the same time requiring much more optimization steps to meet the thresholds, as compared to other websites. 
%Figure \ref{f:ei-emu}(b,e) present the CDF for PLT comparison when optimal configuration is compared with best configuration. Since BO is not guaranteed to find the best possible configuration, there are cases where best configuration has not been explored by BO and the thresholds are met. Tuning the threshold allows BO to find the best configuration but requires much more optimization steps.
%Figure \ref{f:ei-emu}(c,f) present the CDF for number of optimization steps required. 3 is the minimum number of optimization steps required, since after 3 optimization steps the threshold min\_sample\_tested=8 is reached with init\_samples=5. 
%
%
%%\begin{figure}[tbh!]
%%	\begin{center}
%%		\includegraphics[width=3in]{fig/plt-def-emu-36-5.png}
%%		\caption{CDF of PLTs in emulations -- Default vs Optimal}
%%		\label{f:bo_emu_def}
%%	\end{center}
%%\end{figure}
%%
%%\begin{figure}[tbh!]
%%	\begin{center}
%%		\includegraphics[width=3in]{fig/plt-best-emu-36-5.png}
%%		\caption{CDF of PLTs in emulations -- Best vs Optimal}
%%		\label{f:bo_emu_best}
%%	\end{center}
%%\end{figure}
%%
%%\begin{figure}[tbh!]
%%	\begin{center}
%%		\includegraphics[width=3in]{fig/opt-steps-emu-36-5.png}
%%		\caption{Number of optimization steps required to reach thresholds in emulation}
%%		\label{f:bo_emu_optstep}
%%	\end{center}
%%\end{figure} 
%
%\begin{figure}
%	\centering
%	\begin{subfigure}[b]{0.55\textwidth}
%		\includegraphics[width=3in]{fig/combined-emu-142-5-full.png}
%		\caption{EI = 5\%}
%		\label{f:ei-5} 
%	\end{subfigure}
%	
%	\begin{subfigure}[b]{0.55\textwidth}
%		\includegraphics[width=3in]{fig/combined-emu-142-10-full.png}
%		\caption{EI = 10\%}
%		\label{f:ei-10}
%	\end{subfigure}
%	\caption{Effects of EI on optimization steps and optimality}
%	\label{f:ei-emu}
%\end{figure}
%
%
%\textbf{Effect of thresholds on final configuration:} The thresholds controls the trade-off between exploration and accuracy. A lower EI threshold might lead to a better configuration but would require additional search time and optimizations steps. To quantify the affects of Ei, we run BO emulations with different EI values. Figure \ref{f:ei-emu} presents the results for EI=5\% and EI=10\%. A sit can be seen, there is a significant decrease in number of optimization steps required by using EI=10\%. There isn't a significant loss performance benefits by using EI=10\%. The BO-recommended configuration is still performing much better than default and performing within 3\% of best configuration for majority of websites in the median case.



%\subsubsection{Best configuration vs Default configuration}
%The Figure~\ref{f:bestvsdefault} presents CDF of PLT comparison for default versus best configuration case in all network conditions explored in experiments. As can be seen from graph PLT, reconfiguring the networking stack can result in as much as 60\% improvement in PLT.
%

%\subsubsection{Subset of best configurations}
%The number of best configurations is very important as it bounds the extent of kernel reconfiguration required. Smaller the number of best configurations, the lower will be the number of sidecars or VMs needed. A question arises: Can we find a set of N configurations such that it can cover M percent of all conditions? This question is crucial since lower the size of N, lower will be the need to reconfigure kernel. It can be easily seen that N and M are directly proportional to each other i\-e greater the size on N, higher the coverage of network conditions (M). In other words there is a trade-off; we would like the N to be small but that would reduce the coverage.

%\subsubsection{Why top 1\% configurations?}
%In order to answer the question discussed in previous paragraph, we considered two cases for each network condition: the single best configuration and the set of top 1\% configurations (having PLTs within 1\% of nest configuration PLT). We depict the relation between the default, the best and the top 1\% in Figure~\ref{f:comp_top_def}. The blue dots represent PLT of default configuration. The red lines are the ranges from lowest PLT of top 1\% (in other words, the best configuration) to the highest PLT. Since both these PLTs are so close to each other, the red lines appear to be red dots in the plot. The lowest PLT of top 1\% (the best configuration PLT) will always be lower or equal to default PLT, equal in the case when default PLT is itself the best configuration. Let us compare the highest PLT of top 1\% to default. 
%
%As it can be seen from the Figure~\ref{f:comp_top_def}, the top 1\% perform better than the default one in almost all of the cases, 97.2\% of cases to be precise. In other words, PLT of any configuration from top 1\% will be lower than that of default case in 97.2\% of all network conditions. In the rest of 2.8 cases, the highest PLT of top 1\% is higher that default PLT by a mean of 40 ms. Note that although the highest PLT of top 1\% is higher that default PLT in 2.8\% of situations, it does not mean that the corresponding configuration will be selected. Selection of configuration entirely depends on the subset of configurations selected, in other words the size of N discussed in previous section.
%
%%22, 2.86
%\begin{figure}
%	\begin{center}
%		\includegraphics[width=3.2in]{fig/comp_top_def.png}
%		\caption{PLTs for Default vs lowest and higest of top 1\%.}
%		\label{f:comp_top_def}
%	\end{center}
%\end{figure}



%\subsubsection{Number of best configurations}
%Figure~\ref{f:bestvsdefault} shows CDF without taking into account the cost of reconfiguring network stack. Surely reconfiguring the stack will take some amount of time. No matter how small it is, it will be a performance hit. This section expands on finding a set of configurations that can help in majority of the cases.


%\subsubsection{N configurations to rule them all:}
%Finding a small set of configurations that benefit majority of cases is crucial since it will reduce the frequency of reconfiguring network stack in kernel.
%
%In order to find the N configurations, we convert our dataset into M disjoint graphs. Each graph represents a specific network conditions, whereas, the collection of nodes represents the set of top 1\% configurations. We need to find a set of configurations such that each graph contains atleast one node from this set. Using this representation, finding N configurations becomes an instance of set-cover problem.  
%
%Figure~{f:cdf} shows a CDF of configuration coverage i-e the percentage of network conditions a specific configuration performs among the top 1\% of the available configurations. 
%
%\begin{table*}[tbh!]
%	\begin{center}
%		\begin{scriptsize}
%			\begin{tabular}{|c|c|c|c|c|c|c|}
%				\hline 
%				Key&TCP congestion&Initcwnd&autocorking&low\_latency&slow\_start\_after\_idle&pacing\\\hline
%				C1 & Reno & 16 & 1 & 1 & 1 & 0 \\
%				 & Vegas & 12 & 0 & 0 & 0 & 1 \\
%				 & Vegas & 4 & 0 & 0 & 0 & 1 \\ \hline
%				C2 & Reno & 20 & 1 & 1 & 1 & 0 \\ 
%				& Reno & 20 & 1 & 0 & 1 & 0 \\
%				& Cubic & 12 & 1 & 1 & 0 & 0 \\ \hline
%				C3 & Reno & 20 & 1 & 0 & 1 & 0 \\
%				& Cubic & 16 & 0 & 0 & 1 & 0 \\ \hline
%			\end{tabular}
%		\end{scriptsize}
%	\end{center}
%	
%	\caption{Configurations for decison tree}
%	\label{t:dtree-configs}
%\end{table*}
%
%
%
%\begin{figure}[tbh!]
%	\begin{center}
%		\includegraphics[width=3in]{fig/coverage-aws.png}
%		\caption{CDF for network coverage}
%		\label{f:cdf}
%	\end{center}
%\end{figure} 


%In order to find the N set of configurations that can help in majority of cases, Figure~\ref{f:cdf1} and \ref{f:cdftop1} are drawn. Figure~\ref{f:cdf1} shows a the number of configurations on x-axis and percentage of network coverage on y-axis. Figure~\ref{f:cdftop1} presents the same CDF for top 1\% case. The same trend can be seen in these figures as in Figure~\ref{f:cdf} and \ref{f:cdftop}. Slope fop top 1\% is steeper than for best configuration. 
%The following table~\ref{t:covper} shows the N for 70\%, 80\%, 90\% and 95\% coverage on network conditions. The top 1\% case clearly helps in reducing N to much smaller number without losing much in performance as discussed previously.  
%
%\begin{table}[ht]
%	\begin{center}
%		\begin{scriptsize}
%			\begin{tabular}{|c|c|c|}
%				\hline 
%				\textbf{Coverage} & \textbf{N for Best config.} & \textbf{N for Top 1\% config.} \\ \hline
%				70\% & 39 & 19 \\ \hline
%				80\% & 50 & 29 \\ \hline
%				90\% & 69 & 46 \\ \hline
%				95\% & 84 & 57 \\ \hline
%			\end{tabular}
%		\end{scriptsize}
%	\end{center}
%	
%	\caption{Number of configurations(N) for different coverage percentages.}
%	\label{t:covper}
%\end{table}
%
%\begin{figure*}
%	\begin{center}
%		\includegraphics[width=\textwidth,height=5cm]{fig/cdf_v1.png}
%		\caption{Number of configurations needed to reach a specific percentage of coverage (Best configuration case).}
%		\label{f:cdf1}
%	\end{center}
%\end{figure*}
%\begin{figure*}
%	\begin{center}
%		\includegraphics[width=\textwidth,height=5cm]{fig/cdf_v1_logscale.png}
%		\caption{Number of configurations needed to reach a specific percentage of coverage (Best configuration case).}
%		\label{f:cdf1}
%	\end{center}
%\end{figure*}
%
%
%\begin{figure*}
%	\begin{center}
%		\includegraphics[width=\textwidth,height=5cm]{fig/cdf_v1_top.png}
%		\caption{Number of configurations needed to reach a specific percentage of coverage (Top 1\% configuration case).}
%		\label{f:cdftop1}
%	\end{center}
%\end{figure*}
%\begin{figure*}
%	\begin{center}
%		\includegraphics[width=\textwidth,height=5cm]{fig/cdf_v1_top_logscale.png}
%		\caption{Number of configurations needed to reach a specific percentage of coverage (Top 1\% configuration case).}
%		\label{f:cdftop1}
%	\end{center}
%\end{figure*}



%\subsection{Wide Scale Deployment}
%To quantify the benefits of \sysname under realistic and dynamic conditions, we deployed \sysname on Amazon Web services and used deployed client software on a combination of PlanetLb~\cite{} nodes and volunteer servers. For the client software, we developed a framework in python using Selenium and PhantomJS. This client framework allows us to load websites while capturing relevant metrics: PLT and SpeedIndex.  We configured each client to periodically request each website every XX hours.

%\subsection{Learning Speed} 
%\sysname explores the use of multiple techniques to learn optimal set of configurations for a client. 
%
%\textbf{Naive Learning:} From our AWS deployment of \sysname and PlanetLab clients, we have data of around 850,000 page loads. Since our test-bed deployment uses a round-robin approach for routing client requests to differently configured back-end servers, we have PLT data for hosted websites from PlanetLab. By comparing the PLTs, the set of best configurations for a specific client can be figured out. 
%
%\textbf{Decision Trees:} 
%Figure~\ref{f:dtree} shows decision tree for one of the websites from our data-set. This decision tree is built upon the data from AWS tests. As input it takes, client's network conditions (bandwidth, loss rates and RTT) and decides the optimal configuration for the specific client. A separate decision tree is built for each of the website.  
%
%\begin{figure}[tbh!]
%	\begin{center}
%		\includegraphics[width=3in]{fig/stackoverflow.png}
%		\caption{Decision tree for stackoverflow}
%		\label{f:dtree}
%	\end{center}
%\end{figure} 

==> oldlearning.tex <==
\section{Old Learning}
\begin{equation}
P = \{ f (c, n, w) | \forall  c \in C, n \in N, w \in W  \}
\end{equation}
We are interested in finding \textit{c\textsuperscript{*}} such that:

\begin{equation}
min (P) = f (c^*, n', w')
\end{equation}
respectively while \textit{n$'$} and \textit{w$'$} represents a specific case. The size of \textit{W} is under website operator's control, whereas the size of \textit{N} can be virtually infinite.
\theo{I can understand why P is expensive to compute, it requries you to iterate through all combinations.  However, why is f() expensive to compute? f() is only over a specific instance} The black-box and expensive to compute nature of \textit{f()} makes it hard to find the utility of a certain \textit{c$'$}. \theo{How is the utility of a certain c$'$ defined? if f() is all you need to find the utility of c$'$, then this is easy. } It requires changing the networking stack configuration of the server and getting the performance metrics from the user. In a productin enviroment, this can adversly affects user's QoE. Hence, the size of \textit{C} is bounded by the extent to which a user can be put through the variations in QoE. \theo{why does the extend to which a user can be put through variations bound the size of C? I'm potentially missing something crucial here.  I don't believe our value of C is bounded by any of this} Its size is also bounded by a user-defined threshold on improvement in performance. \theo{What user-defined threshold? In theory, we can add an extension to Chrome to capture this input, but this is not that practical.} This threshold directly relates to the optimality of the configuration (whether its the best we can find or just good-enough).

	
\textbf{A/B tests:} The live performance collection from end-users makes A/B testing a suitable contender for \sysname. \theo{Why?  is A?B a suitable contender? what about the properties of A/B or the live performance collection make A/B a suitable contender?} A/B testing has been vastly used in solving similar black-box functions~\cite{kraken, tcpwise}. The basic idea is to use different confiurations for a user and then compare their performance. Its a closed-loop system that operates on live traffic to estimate the utility of a configuration. Using live traffic makes the system adaptable to changes in underlying network conditions and have an updated view of the workloads. The feedback loop starts at server picking a certain user for A/B and reconfiguring the network stack for that user. It ends at collecting the user's performance and network condition metrics.
 Three important questions arise:
\begin{itemize}
	\item What's the next user to choose? In production environment, there can be thousands of users to choose from. Selecting every user for A/B is a bad idea as it can adversely affect user's QoE.
	
	\item What's the next configuration to test in A/B tests? Choosing a wrong configuration will have a bad affect on user's QoE.
	
	\item When to stop the A/B tests for a previously selected user?
\end{itemize}

\theo{By definition optimal should be best -- you can't do better than optimal or best. If we aren't going to use optimal as best, then we need to use a different word.}
\textbf{Objective:} The objective of our learning model is to find an optimal configuration, where it is defined as the configuration performing better than the default one. Note that, optimal configuration might not be the best configuration available. Also there might be cases when the default, optimal and best configuration can be the same ones.

\textbf{Strawman solution}
A naive solution is to use random sampling. A user is random selected at the beginning of a connection and a random configuration from the superset \textit{C} is assigned to her. Random sampling has been used with success in past \cite{kraken, tcpwise}. If the randomly-sampled configuration works better than the previous configuration, the optimal configuration for the user is updated. 

\theo{Why does random sampling miss history? Kraken has some historical information build it. It doesn't use history to do any prediction but it may have some naive learning.}
Random sampling misses one important aspect, it doesn't take historical data into consideration while making sampling decisions. \sysname presents a better solution for the questions asked above by taking into consideration what we already know about a user.

\subsection{Learning  the optimal configuration in \sysname}
%\subsection{\sysname feedback loop design overview}
\theo{where does learning fit in the feedback loop?}
In this section, we present two approaches that \sysname use for learning the optimal configuration; machine learning and statistical learning.

\theo{This repeats what was said earlier and makes uses the terms best/optimal in a questionable way.}
\textbf{Best vs optimal configuration:}
Finding the best network stack configuration is difficult due to the following challenges:

\begin{itemize}
	\item Finding the best configuration requires an exhaustive search of the complete configuration space, which is time consuming. 
	\item An exhaustive search requires continuously reconfiguring the networking stack. From a production system's point of view, this is infeasible as a bad configuration can adversley affect enduser's QoE. Content providers do not want that as Google reports that increasing search latency 100 to 400 ms results in a 0.2\% to 0.6\% reduction in number of searches per user.
	%	http://services.google.com/fh/files/blogs/google_delayexp.pdf
	\item The diversity in network conditions and webpage complexity makes this even more difficult, as they affect the performance of a configuration and content providers do not have a control over underlying network conditions.
\end{itemize}

Due to these challenges, we relax the objective from best configuration to optimal configuration, where optimal configuration is defined as a configuration that works the same or better than default configuration. The extent of improvement of optimal over default varies from case to case. There can be cases when both optimal and best configurations are identical. On the other hand, optimal and default configurations can be the same for the scenarios where we cannot find a configuration performing better than the default one.

\textbf{Machine learning approach:}
\theo{why random forest? and not some other learning?  the stream processign did a good job of comparing and discussing a range of other approaches.}
In the ML version, \sysname uses Random Forests \cite{} to learn the optimal configuration for a user. Using A/B tests, performance data for different configurations  is collected and the configuration with the least latency is selected as the optimal configuration for a specific user.  A random forest is trained on the collected data, which is then used for predicting the optimal configurations for other users.\theo{what is the feature set? What parametesr are used for the random forest?}

\textbf{Statistical learning approach:}
\theo{Why BO? what are the other options?}
In the SL version, Bayesian Optimization(BO) \cite{} is used for predicting the optimal configurations. BO is an effective global optimization startegy, especially for black box functions. Our objective is to minimize the latency for a user and we dont know about the internals of objective function specied in eq. 1 and 2. This makes BO a contender for solving the optimization problem of finding the configuration with least latency. BO treats the unknown objective function as a random function and place a prior function over it. The prior function is expected to capture our beliefs about the objective and what the actual values might look like. The prior function incorporates posterior probability distribution of the unknown objective functions outcomes. The objective function is observed through experiments and the collected performance data is used by BO to improve the posterior probability distribution over the objective function. We use Gaussian Process \cite{} as the prior function and Expected Improvement(EI) as the acquisition function, due it its effectiveness in related works \cite{cherrypick, ituned}.

Our objective function has all the classical properties of that BO specializes in. \theo{is there a citation for classical properties?} The function is expensive to evaluate. Its derivative information is not available and dimensions are not too large. \cite{}
 
 *** I think a figure about BO, confidence interval and acq function is needed here. ***
 
In the following paragraphs, we expand on the various components in \sysname's feedback loop using both approaches. \theo{which following paragraphs? the feedback loop only had two things: pick user and collect data. where does ML}

\theo{We need more context before we can jump into the next few sections}
\subsubsection{Clustering users by network conditions}
The feedback loop starts at picking a user for A/B tests. However, since \sysname makes this decision by taking the historical data into account, it needs to have an idea abpout the network conditions faced by the user. \sysname actively collects performance metrics and network condition statistics about every user it interacts with (later explained in Section \ref{s:archi}). These statistics allow us to keep track of user's network conditions and use them for making any decision. Whether its SL or ML, these colected statistics are the basis features for learning optimal configurations.

Users with similar network conditions should have similar optimal configurations. This highlights the importance of picking the right cluster for a user since \textit{what's learnt for one user can be used for another one if they belong to the same cluster}. This greatly alleviates the hurdle of learning for an inifinite combination of network conditions to a lmited number of clusters, that are pre-defined. From our experience with \sysname, we have found that picking the right sizes for the clusters is integral for any kind of subsequent learning. 

\theo{what is the right cluster size? how did we pick this?

If the clusters are fine-grained, this would improve learning accuracy as the cluster will contain users who are very similar to eachother. If the clusters are too large, diverse users are clustered together, making the learning model to under-fit as minority results (corner cases) will be shadowed by majority ones. On the other hand, fine-grained clusters lead to lower number of performance data samples in each cluster, that reduces learning accuracy. Hence there's a tradeoff between cluster sizes and the dergree of exploration. \sysname uses measurments from Facebook, Google and Verizon as basis for selecting the right cluster sizes \cite{facebook-network-classification, verizon-report, wpt-figure}. \theo{How do we use this data for decising cluster? are these really clusters as in Machine learns for just predefined buckets?} The cluster sizes cover a wide range of diverse network conditions and keeps the cluster sizes to the minimum, without sacrificing too much degree of exploration.

\begin{figure}[tbh!]
	\begin{center}
		\includegraphics[width=3in]{fig/NetworkConditions.png}
		\caption{network conditions}
		\label{f:net-conditions}
	\end{center}
\end{figure}

\subsubsection{Initial configuration sampling}
\sysname needs some initials configuration samples to bootstrap the learning process. Hence initially, \sysname uses configuration sampling to assign a certain configuration to a user. \theo{where does this fit in the feedback loop?}

Except ICW, all of configuration parameters under consideration are categorical (eg, HTTP either 1 or 2, tcp\_autocorking either 0 or 1). This reduces the sample space for the number of available configuration combinations. Instead of using a range of continuous whole numbers for ICW, we divide it into intervals to reduce the ICW search space. We have tested with various intervals and an interval of 5 is found to be suitable. \theo{there are no results for this testing. Do we have them anywhere?}

\theo{this next sentence is a rewording of the initial sentence in this subsubsection}
At the beginning, \sysname needs initial data points for building learning model (either BO or RF). Random sampling is found to be effective in some recent work \cite{cherrypick}. \sysname build on random sampling by using domain heurictics to improve randomness. \sysname uses the knowledge about a user's network class for sampling initial configurations to be tested. \theo{What is a network class? who defines it? is this the cluster above?} Since we have some estimate of a user's network conditions, we can use these estimates for improving random sampling by fitting it to the user's case.  

\begin{itemize}
	\item \textbf{ICW:} \sysname looks at user's previously mesured \textit{slow start threshold(ssthresh)} value and picks an ICW lower than that. \textit{ssthresh} provides an active view of bottleneck link capacity between client and user, which is used for estimating next ICW to be tested. \theo{this is not random, or close to being random.}
	\item \textbf{HTTP:} A lot of work has been done to understand the affects of network conditions on HTTP versions \cite{spdy, other}. \sysname leverages these studies for selecting HTTP version. \theo{How?}
\end{itemize}

\theo{There is no use fo the word random in this paragraph. Instead of random, we use domain knowledge to rank and then pick based on this ranking. Do we evaluate the implication of using this ranking against a truly random selection.}
We extend the heurestics to the other configuration parameters by leveraing the data collected from active experiments. Using the test-bed described in Section \ref{s:motivation}, we performed in-the-wild experiments between AWS servers and PlanetLab clients, where we explored the entire configuration space and evaluated its performance. Once we have measured the perofrmanc of different configurations in diverse network conditions, we can rank the configurations according the their utilites. \theo{this doesn't not seem random.} Utility in this context is defined as the percentage of network conditions in which a certain network configuration proves to be optimal. Thus by ranking the configurations by their network coverage, initial sampling can be refined, since a configuration with higher network coverage has a higher probability of being the optimal configuration in an unseen network condition. This tremendously reduces the configuration space to be explored, since if the threshold on improvement is reached within the first highest-ranked configurations, \sysname does not need any more configuration sampling. Otherwise, ICW and HTTP heuristcs are used and the other parameters are sampled randomly. 

%Figure \ref{f:subopt} summarizes the results from the experiments by plotting a sub-optimality curve. Sub-optimality is defined as the comparison between N configuration set PLT and default configuration PLT, when one of N configurations is used for the entire experiment space. An interesting conclusion that can be drawn from the plot is that for N as small as 6, sub-optimality is zero for around 72\% of the cases. In other words, for 72\% of the cases, N contains a configuration that is better than the default one. This tremendously reduces the configuration space to be explored. Consequently, initial configuration sampling uses the N=6 set as the basis. If the threshold on improvement is reached within this set, \sysname does not need any more configuration sampling. Otherwise, ICW and HTTP heuristcs are used and the other parameters are sampled randomly.

%\begin{figure}[tbh!]
%	\begin{center}
%		\includegraphics[width=3in]{fig/subopt_pl_v1.png}
%		\caption{Sub-optimality of using N network configurations}
%		\label{f:subopt}
%	\end{center}
%\end{figure}

%\subsubsection{To A/B or not to A/B}
\subsubsection{Selecting a user and configuration for A/B}
\theo{when is the intial data collected? when is the next used?}
Once the user is classified into one of the clusters, \sysname uses learning model and historical data to decide whether to flag the user for A/B or not. We present two strategies for this:

\textbf{SL:} The nice thing about the use of Bayesian Optimization for black-box functions is the presence of \textit{acquisition function}. BO build the acquisition function using the posterior probability distribution. Acquisition functions estimates the outcome of the balck-box function at a certain input, using the probability distribution built using input data. In other words, it tells us about the next data point to explore. \sysname SL uses its acquisition function to determine the next configuration and its expected outcome. If the expected improvement(EI) is higher than user-defined threshold, the user is selected for A/B test. 

\textbf{ML:} The network class of newly-connected user is fed into random forest model and the model predicts a suitable configuration, based on the trained data. However, we still need to decide whether to pass the user through A/B test or not. 

A random forest(RF) is a collection of decision trees with varying feature sets. When RF predicts a configuration for a network class, it gives back the configuration, elected by the underlying decision trees. In other words, we can use these votes as a measure of prediction strength. If a prediction is strong enough, we are confident that the configuration is optimal. If the votes are divided, the prediction  might not be strong enough and its an indication that we need more data observations for that specific network class. Hence for every network class, if the majority vote is less than a user-defined threshold, the user belonging to this network class are selected for A/B tests. This leads to incresed number of data points for the specific network class, resulting in swaying the votes in one direction.

After a user is selected for A/B by voting, one of the initially sampled configuration for the network class is assigned to the user.
 

\subsubsection{Performance feedback and model creation/update}
The next step is to collect the performance metrics for the new configuration and update the underlying learning function. At this step, we have performance metric(eg, PLT) of a certain configuration for a user(belonging to a certain network class). The implementation of the performance collection process is explained in Section \ref{s:archi}.

\textbf{SL:} SInce network conditions govern the performance of a configuration, it would be unwise to use a single, collective BO model for all network classes. This would lead to serious problems as a single configuration can have different performance in different network conditions, eg, high ICW in low bandwidth can lead to losses and retransmissions, resulting in higher PLT. As a result a different, separate BO model is developed for each network class. Once the performance metrics have been collected for the configuration specified by acquisition function, the new observations are fed and the model is optimized to incorporate the new findings. This leads to improvement in posterior probability distribution. \theo{will all SL have multiple models?}

\textbf{ML:} A single RF is developed which takes network classes as feature set to predict optimal configuration. With new observations, the RF model is incrementally updated to incorporate new findings. \theo{Will all ML have a single model? }

This marks the ending of feedback loop. The outcome is more observed data points, which naturally leads to improvement in accuracy. 


\begin{table*}[tbh!]
	\begin{center}
		\begin{tabular}{| p{3cm} | c | p{4cm} | p{4cm} |}
			\hline 
			\textbf{Paper} & \textbf{Initial sampling} & \textbf{Optimization/learning} & \textbf{Termination condition} \\ \hline
			CherryPick & Quasi-random sampling & Bayesian optimization & \{EI, no. of samples\} threshold \\ \hline
			iTuned & LHS & Gaussian process (GRS) & EI threshold \\ \hline
			BestConfig & LHS & Hill climbing & resource budget \\ \hline
			Tuning of Stream Processing Systems & mLHS or random & modified hill climbing or rule-based & resource budget \\ \hline
			TCP WISE & random & statistical modelling & Time threshold \\ \hline
			ConfigTron SL & random with heuristics & Bayesian optimization & \{EI, no. of samples\} threshold \\ \hline
			ConfigTron ML & random with heuristics & Decision Trees & no. of samples threshold \\ \hline
		\end{tabular}
	\end{center}
	\caption{Configuration learning in related works}
	\label{t:learning-related}
\end{table*}





%0- Choice of bucket
%1- Affect of bucket sizes from our experience, Facebook, WPT, Verizon citation
%2- A tradeoff between learning speed and accuracy
%
%1- Initial sampling
%LHC (or random) with custom heuristics 
%
%2- Learning function
%SL vs ML
%
%3- Picking the next run for A/B
%1- In SL, acquisition functions
%2- In ML, voting by number of samples in leaves
%
%4- Stopping Criteria
%1- In SL, bound on EI
%2- In ML, bound on number of samples in respective leaf
%
%5- Scalability
%1- In SL, one BO model per network condition.
%2- In ML, one decision tree
%
%6- Speed of collecting measurement/performance data

%\subsection{Data pre-processing}
%In order to feed our data set to the learning function, we first process the data to format the data in suitable format. The features on which we learn our model comprises of bandwidth in bytes/sec, RTTs in ms, packet loss rates and websites/origin webserver. The first step in data pre-processing is to extract targets for the corresponding features from the data set. Due to in-the-wild nature of experiments, the combinations for bandwidth, RTT and loss rates can be virtually infinite. In order to find the most optimal configuration in a certain network scenario, we divide the observed network conditions into buckets. In each network condition bucket, we compare PLT of a certain website to judge which of the configuration works the best. The configurations whose PLT is within 1\% of the least observed PLT in the certain bucket is selected to be the optimal configuration. Selecting the right bucket size is critical to learning. If the bucket size is too small, it might cover very few data points. On the other hand, too large buckets can make our learning model to under-fit as minority results (corner cases) will be shadowed by majority ones. From our experiments we have found 10kB/s for bandwidth, 0.1\% for packet loss and 10ms for RTT to be the best bucket sizes. 
%Another direction that we are pursuing for bucket size is to cluster the features using k-means, where k is determined by the comparing mean squared errors.
%
%\subsection{Decision trees}
%Uding the data generated from test bed, we used decision trees as our learning function. Using Gini Impurity as our criterion function and 2 as the minimum number of samples required to split an internal node we were able to get as high as 96.65\% accuracy. We used 10\% of our initial data set as test data and the rest as training data for the decision trees.
%
%\subsection{SVM}
%
%
%\subsection{Clustering}
%
%
%\subsection{Neural Nets} 
%
%
%\subsection{Genetic Algorithms}



==> overheads.tex <==
\subsection{MicroBenchmarks}
\label{s:overheads}
We conclude by analyzing the impact of the \agent on a web server. Specifically, we explore CPU and memory overheads of \agent and the performance implications of having \agent interpose on each connection.  We conducted these tests using \AB tool~\cite{ab} between a local \sysname-enabled server and a local client running the \AB tool. We repeated tests in multiple network conditions, with multiple number of concurrent connections and for multiple websites.
%We omit our results due to space limitations and present a summary below.
% In these experiments, \AB is configured to generate 100 concurrent requests and each experiment is run 10 times to eliminate variations.

%overheads: CPU utilization, memory utilization, server throughput and latency.  To conduct these tests, we leverage the Apache Benchmark tool~\cite{} (AB) and focus on controlled experiments in our testbed which allows us finely control networking and server conditions.

\parab{Overheads:} We compared \sysname against a vanilla server using \textit{Cubic} (default setting). To keep comparison fair, \sysname was tuned to use \textit{Cubic} for each connection. AB benchmarking showed no overhead of using \sysname's kernel module in term of latency. Similarly, we did not observe any CPU and RAM (less than 1\%) overheads. Any RAM overhead is attributed to kernel module's implementation of KV-store \cite{}, used for storing IP masks to configuration rules..

%\parab{Resource Overheads:} 
% \textbf{Takeaway:} \sysname incurs no additional overheads in terms of latency RAM or CPU. We also plan to explore the use of eBPF and XDP as methods for further improving its interoperability.

%To better understand the overheads contributed by \agent code and to separate these overheads from those contributed by the underlying call interposition framework, i.e., $LD\_Preload$, we compared \sysname against a vanilla web server (BaseLine) and a web server with $LD\_Preload$ used to interpose on sockets calls but the interposition code does no additional processing or reconfiguration.  
%Figure~\ref{f:ab1} presents the throughput and latency measurements. 
%We observed that while \sysname reduces the server throughput by 12.4\%, simply using $LD\_Preload$ already created a 9.5\% server reduction in throughput. This indicates that we may be able to improve \sysname by exploring alternative methods for interfacing the \agent with the web serving stack. 
%We observed that \sysname inflates the mean latency by ~2.2\% over that of $LD\_Preload$ (2.2\%).


%In order to measure the overheads of using using \sysname, we performed AB tests in three experimental scenarios, (i) Using LD\_PRELOAD to reconfigure apache (as in \sysname), (ii) Using LD\_PRELOAD to wrap accept() system call and (iii)
%unmodified Apache. The second comparison quantifies the overheads of using LD\_PRELOAD. Here LD\_PRELOAD directly calls accept(), without any reconfiguration to TCP parameters. We used a client in AWS and tested a total of 1000 requests in each turn, keeping 100 as the concurrent number of requests. Every measurement is performed 10 times to cater for the variation and the outliers are filtered.
%To keep the measurements realistic, we use PlanetLab \cite{} nodes as clients. Starting with a single client running AB tests, we keep increasing the number of clients till it reaches one hundred. Each client makes 10 requests, keeping five as the number of concurrent requests per client. All measurements are taken using a server running on an Intel Xeon processor (12 cores @ 2.0GHz) with 16GB of RAM, running Ubuntu 14.04 Linux 3.13.0-105-generic OS. Clients are PLanetLab nodes running on Intel Xeon, 4GB of ram and running Linux 2.6.32 OS. 
%Figure~\ref{f:ab1} compares throughput for the three scenarios. Using LD\_PRELOAD results in 9.5\% decrease in throughput as compared to unmodified Apache whereas using ConfigTron results in 12.4\% decrease in throughput.  
 
% \begin{figure}[tbh!]
% 	\begin{center}
% 		\includegraphics[width=3in]{fig/throughput.png}
% 		\caption{Throughput comparison}
% 		\label{f:ab1}
% 	\end{center}
% \end{figure}
% \begin{figure}[tbh!]
% 	\begin{center}
% 		\includegraphics[width=3in]{fig/time_benchmark.png}
% 		\caption{Latency comparison}
% 		\label{f:ab1}
% 	\end{center}
% \end{figure}
%
% \theo{Currently, we don't say anything about these latency graphs.}
% Figure~\ref{f:ab2} shows the latency comparison of the three scenarios. The plot shows percentage of the requests served within a certain time. As expected unmodified Apache works the best, followed by LD\_PRELOAD version, and then \sysname.
%


%\parab{Resource Overheads: } %Next, we analyze the resource overheads of the \agent. 
%We observe that \agent used less than 5\% additional memory and CPU. %The minimal resource overheads are due to the lightweight nature of the \agent.
%
%\textbf{Takeaway:} \sysname incurs small overheads and we plan to explore the use of eBPF and XDP as methods for further reducing these overheads.
%
% In order to quantify  the performance implications of \sysname, we monitored the server's RAM and CPU usage under heavy load (From 50 to 500 concurrent connections). As far as CPU utilization is concerned, using \sysname result in a increase in CPU utilization as compared to native apache due to background TCP monitoring and learning. \theo{why is learning causing a problem? for background TCP monitoring we are using the TCP-stucture, how much of the processing is due to the usage of this struct?}Figure~\ref{f:ab4} and \ref{f:ab5} gives a comparison of RAM and CPU usage usage. \sysname requires background monitoring of TCP flows and building/updating the learning which adds to memory and CPU usage. We have kept background monitoring as light as possible by keeping it single-threaded iterating over an array of active sockets.
%
% \begin{figure}[tbh!]
% 	\begin{center}
% 		\includegraphics[width=3in]{fig/ram_comparison.png}
% 		\caption{Ram usage comparison}
% 		\label{f:ab4}
% 	\end{center}
% \end{figure}
%
% \begin{figure}[tbh!]
% 	\begin{center}
% 		\includegraphics[width=3in]{fig/cpu_comparison.png}
% 		\caption{CPU usage comparison}
% 		\label{f:ab5}
% 	\end{center}
% \end{figure}



==> prelim.tex <==
\section{Prototype Implementation}
To explore the feasibility and viability of \sysname, we have developed an initial prototype and are exploring the implications of employing it on a cluster of 300 servers and also on Amazon EC2 using PlanetNodes as clients.

% In fact, our prototype implementation was used to develop the results in Section~\ref{s:archi}.

\textbf{Implementation Highlights}:

%\theo{How many lines of code?}
\begin{itemize}
	\item Config Agent: We have implemented the Config agent in Python in 890 lines of code. The Config agent provides controls over the configuration parameters discussed in Section~\ref{s:motivation}.  The Config agent transmits configuration profiles to the ConfigProxies using simple RPC requests.
	\item Request Router: The request router is implemented using IPTables. We NAT Src IP-prefixes to different ports. The ConfigProxies in turn bind to these different ports allowing them to receive/send these packets.
	\item Sidecar: Encapsulates the different ConfigProxies and is implemented using XXX.
	\item ConfigProxies: The ConfigProxy is developed atop the cURL~\cite{} proxy library and bound to a pre-specified port and on startup it receives config profiles form the ConfigAgent and appropriately configures its ports using the appropriate low-level commands.
	 
\end{itemize}

% \begin{figure}[tbh!]
% 	\begin{center}
% 		\includegraphics[width=3in]{fig/socket1.png}
% 		\caption{System Architecture}
% 		\label{f:arch1}
% 	\end{center}
% \end{figure}


% Exploring the life cycle of a new request, a new request is forwarded from client to load balancer. The load balancer forwards the request to one of the servers using traditional load balancing algorithms (eg, round robin). If no rule is present in iptables for the client, the request is served using the default network configuration of server (eg, by apache server running at port 80). If a rule is present in iptables matching client's IP, the request is forwarded to a side-car on the same server (eg, socket operating at port 20000). the presence of rule in iptables for a client is indication of the fact that the learning function has previously instructed the local configuration agent to install the rule. As a result of this iptable rule, the request is forwarded to the socket side-car that has the optimal network configuration for the client. Once a request reaches a side-car, it is forwarded to the actual web server (eg, apache) listening at a different port (eg, the default 80 and 443) using proxy operating within side-cars context. The proxy gets the response from web server and the response is sent back to the client using the reconfigured socket of side-car.





%\textbf{Unexpected Challenges} An interesting challenge we faced during the implications and deployed our \sysname is the interactions between our system and L7 load balancers. 

==> randomness.tex <==
\subsubsection{Impact of \textit{Degree of Randomness}}
\label{s:randomness}

% \begin{figure}[tbh!]
%	\begin{center}
%		\includegraphics[width=3.2in]{fig/randomness_plt.eps}
%		\caption{Impact of different degrees of randomness}
%		\label{f:rand}
%	\end{center}
%\end{figure}

% \begin{figure}[tbh!]
%	\begin{center}
%		\includegraphics[width=3.2in]{fig/randomness_box.eps}
%		\caption{Impact of different degrees of randomness}
%		\label{f:rand1}
%	\end{center}
%\end{figure}

 \begin{figure}[tbh!]
	\begin{center}
		\includegraphics[width=3.2in]{fig/randomness_cdf.eps}
		\caption{Impact of different degrees of randomness}
		\label{f:rand-cdf}
	\end{center}
\end{figure}

The \textit{Degree of Randomness} (\S \ref{s:abtesting}) controls the rate of exploration. A higher value leads to more connections sampled for A/B testing, but have the implications of hurting client's performance due to testing a sub-optimal configuration. In figure \ref{f:rand-cdf}, we specifically focus of performance degradation (lower tail) for different values of randomness. A high value (15\%) can lead to degraded performance as compare to Default configuration for 7\% of tail conditions. In \sysname prototype, we went with middle-ground and sampled 5\% of connections for A/B testing.







==> sensitivity.tex <==
\subsubsection{Sensitivity Analysis}
\label{s:sensitivity}
The design of machine learning algorithm is sensitive to algorithm's hyper-parameters and the size of the data set.

\input{traffic_size}

\input{offline-learning}

\subsubsection{HyperParameter analysis}
\label{s:sensitivity-para}
Next, we analyze the impact of the various hyper-parameters on the accuracy and performance of the different learning algorithms.% For each algorithm, we focus here on several key parameters that impact performance.

\sout{
\parab{Clustering Algorithm:} We first analyze the clustering method used to create network classes. We specifically explore two options: first, using k-means clusterings and second, using domain knowledge (e.g. Facebook Network Classes \cite{fbconn}).  We observe that both methods results in data points being placed in roughtly the same clusters: 83.3\% of the connections are binned into the same clusters.
%Kmeans resulted in higher number of clusters, dividing  our network class into two or more. However, for majority of these cases same favorable configuration was being used in both cases. Thus overall, the cluster changed, but configuration remained the same. 
The end result of this similarity is that the learning algorithms, in general, perform virtually identically under both approaches to defining network classes.
}

%For example, in Figure~\ref{f:clustering}, we present results from the \ML algorithm which are presentative. These results highlight that while there are minor difference in the clustering, these are do not significantly impact performance.

% \begin{figure}[tbh!]
% 	\begin{center}
% 		\includegraphics[width=3in]{fig/manual_vs_auto.png}
% 		\caption{Manual vs automated clustering}
% 		\label{f:clustering}
% 	\end{center}
% \end{figure}

%\begin{figure}[tb!]
%	\begin{center}
%		\includegraphics[width=3in]{fig/init-samples.png}
%		\caption{Number of optimization steps required.}
%		\label{f:init-samples}
%	\end{center}
%		\vspace{-0.2in}
%\end{figure}

\parab{Sampling Algorithm:} Next, we analyze the impact of the three dominant sampling algorithms on our learning algorithms. Specificaly, Random Sampling, Domain-specific (ranking-based) sampling and Latin Hypercube Sampling (LHC) \cite{}.  We observe that the sampling methods impact the speed of reaching a near-optimal configuration.  Moreover, \BO is more directly impacted because \BO's makes intelligent decisions based on the results of initial samples, where as \RF does not use the initial samples to make sophisticated decisions. We found LHC to be working best as the initial samples cover a wider range of sample space. We found LHC to reduce number of optimization steps by 2-3X for some cases as compared to Random. For Domain-specific sampling, we ranked the configuration offline and used the top-N configurations as initial samples. It was found to be restricting as the rankings vary widely across NCs.
   
%Thus, in Figure~ \ref{f:init-samples} we focus on the impact of the sampling algorithms on the number of optimization steps.  We focus on the five representative websites of varying complexity levels~\cite{butkiewicz2011understanding} to understand how the choice of sampling impacts websites of different complexity.  
%We observe that in many of the sites using domain specific can speed up \BO, in the median case, by a factor of 2-3X. Moreover, the results are significantly more impressive at the tail where domain specific results in a factor of upto 6X improvement.\theo{the exception is msn. This should be discussed later. Did we only have five websites?}
%\usama{No we have more. we have a total of 16 websites}
%
% \parab{\SL-Specific Parameters:} We focus on EI, the parameter, which balances the need for exploration with model accuracy.  Lower EI values allow for more exploration and can lead to more accurate model. Where as, higher EI speed up the model building process but at the cost of accuracy. We used several EI values in the simulator and observed that a 3\% worked the best. Any higher value resulted in convergence to a configuration far from the optimal one.
%
% \digdeep{What's the tradeoff for setting EI? A low value would explore better but would take a longer time to converge.}

%, in Figure~\ref{f:ei-emu}, we present two representative points: namely 5\% and 10\%. Once again, we analyze both performance and model building speed.  We observe that the higher value, 10\%, is faster (requires less steps), but does not significantly impact performance.  Motivated by this value, we use an EI value of 10\% in our experiments.

% There is a significant decrease in number of optimization steps required by using EI=10\% and at the same time, there isn't a significant loss in performance benefits by using EI=10\%. The BO-recommended configuration is still performing much better than default and performing within 4\% of best configuration for majority of websites in the median case.

% \textbf{\SL} For \SL, we focus on the EI which impacts the algorithm by controlling the algorithms exploration of and defines the ultimate prediction qualitiy of the model.

%  Figure \ref{f:ei-emu}(c,f) present the CDF for number of optimization steps required. 3 is the minimum number of optimization steps required, since after 3 optimization steps the threshold min\_sample\_tested=8 is reached with init\_samples=5.
% The thresholds controls the trade-off between exploration and accuracy. A lower EI threshold might lead to a better configuration but would require additional search time and optimizations steps. 



\parab{D-Tree Parameters:} We explore D-Tree specific parameters: For information gain, we found that using entropy over alternatives (e.g, gini impurity) resulted in the best accuracy. Similarly using 80 as the minimum samples per leaf, as opposed to a range of other values, resulted in the best accuracy as it minimizes over-fitting.
%\sout{Lastly, we explore \RF specific parameters: number of trees (K) and the information gain function.  For the information gain, we found that using entropy over alternatives (e.g, gini impurity) improved accuracy by 3\%.  We tested different numbers of trees from 10 to 100 and found that the 10 is the optimal choice, providing a good balance between accuracy and training overheads.}

%\theo{The difference between 10 and 64 is 0.15\%, I don't think this is enough to use more than 10 trees (Figure~\ref{f:acc-rf}). The information gain is a significant factor where as the size of the trees are irrelevant.}
	
%<<<<<<< HEAD

%\begin{figure}[tbh!]
%	\begin{center}
%		\includegraphics[width=3in]{fig/acc-rf.png}
%		\caption{Accuracy vs number of trees}
%		\label{f:acc-rf}
%	\end{center}
%\end{figure}


% \usama{I agree. I have edited RF description in prototype.}
% \begin{figure}[tbh!]
% 	\begin{center}
% 		\includegraphics[width=3in]{fig/acc-rf.png}
% 		\caption{Accuracy vs number of trees}
% 		\label{f:acc-rf}
% 	\end{center}
% \end{figure}
%
%>>>>>>> 8ef05a14db78011f14d80b6e2495e0f7a629a267




% \textbf{ML: }
% By exploring the hyper-parameter space, we found the set of random forest tuning parameters that served us the best. We used entropy for the information gain as the measure of quality of split, 64 number of trees (k) in the random forest and sqrt(number of features) as the maximum number of features. We did not limit the depth of the trees and used 2 as the minimum number of samples required to split a node. Using information gain instead of gini impurity lead to 3\% increase in accuracy. Figure \ref{f:acc-rf} shows the accuracy for different k. We tested k=10, 25, 50, 64, 100 and found 64 to be the optimal choice.
%
% There are performance implications for using higher number of trees in random forest as this is inversely proportional to time taken to predict a result (higher number of trees lead to waiting for higher number of votes). Moreover, RAM consumption also increases with increasing number of trees.




%
% \textbf{Ranking-based sampling:}
% We compare ranking-based sampling with random sampling to see the benefit of using a pre-defined set of configurations in bootstrapping the learning process in BO. Figure \ref{f:init-samples} presents the number of optimization steps required in both cases for 5 different websites. For 4 of the websites, ranking-based sampling requires 4 optimization steps whereas random sampling requires 5 to 12 samples for the median case. Note that, 4 is the minimum number of optimization steps since we keep init\_sample=5, min\_sample\_tested=8 and 4 steps are required to cross this threshold. A highly ranked configuration has a higher probability of performing near-optimally for an end-user and this leads to the decrease in number of optimization steps. The results are even more impressive for 90th and 95th percentile for websites except msn.com. msn.com is a special case when using a pre-defined set is causing BO to explore more before meeting the thresholds. A look at msn's PLT results illustrates that for msn, highly-ranked configuration does not work near-optimally, and bootstrapping with such a predefined set of configurations leads to higher number of optimization steps. One way to cater for this problem is to use a mixture of ranked and random configurations for bootstrapping.



%Selecting the right network clustering is integral to \sysname. All users in a network class are expected to have similar network conditions and \sysname will predict a single favorable configuration for all the users in a network class. Due to lack of knowledge about client's network condition, \sysname uses developer-defined countries for classifying users according to their network conditions. These boundaries are decided based on Facebook Network Classes \cite{} and Akamai's and Verizon's report about the network connectivity in the different regions of the world.
%We are interested in finding out the implications of using fixed classes. For this we use data recorded from \sysname deployment and cluster the clients' network conditions by using kmeans clustering. K is selected when mean squared distance between centroid and cluster points does not show significant change on increasing k further. Figure \ref{f:clustering} plots the improvement in performance over default when the two different clusterings are used. There isn't a significant difference in performance improvement when manual clustering is replaced by auto clustering.



==> sl_vs_ml.tex <==
\subsection{SL vs ML highlights}
\label{s:sl_vs_ml}

\begin{itemize}
	\item \usama{Although SL provides a more refined way of exploring new configuration as compared to ML due to the use of acquisition function. However, Having a separate BO model for each network class limits its ability to learn cross-class patterns. Whereas ML is able to generalize the patterns learnt from older classes for a new class (\S \ref{s:benefits-sim}).}
	\item \usama{SL outperforms ML only when the number of available data points is small, as evident from our live deployment ($\sim$100 clients).}	
\end{itemize}

%  and merge different classes together if they show the same behavior. 
%In order to compare the two strategies, we look at the simulated sessions to see improvements over time. We look at a new, incoming client and specifically focus on two scenarios: (i) the client is a member of an existing network class (ii) the client does not belong to an existing class. 
%In both scenarios, client's network class is unknown at the first page load (\sysname measures network conditions during the page load) and a sampled configuration is used. However, their behavior diverges in the next page load.

%\textbf{Scenario 1:} (Figure \ref{f:plt_timeseries_old_nc})
%\usama{
%Both SL and ML models are already mature. The new client gets classified into an existing network a class and its learnt configuration is used. The spikes in PLT are due to the random exploration (controlled by randomness threshold). As it can be seen, SL's prediction is less optimal than ML. Zooming into the results showed that EI threshold is reached before SL has found the optimal one.
%}
%
%\textbf{Scenario 2:} (Figure \ref{f:plt_timeseries_new_nc})
%\usama{
%Since ML is able to learn across network class boundaries, it is able to make use of patterns learnt in other nerwork classes to better predict a good configuration. Whereas SL creates a new BO model for the new class and initiates the learning phase for the specific class by testing random configurations.
%}

%\begin{figure}[tb!]
%	\begin{center}
%		\includegraphics[width=3.2in]{fig/plt_timeseries_new_nc.png}
%		\caption{PLT timeseries -- Scenario 1}
%		\label{f:plt_timeseries_new_nc}
%%		\vspace{-0.2in}
%	\end{center}
%\vspace{-0.2in}
%\end{figure}
%
%\begin{figure}[tb!]
%	\begin{center}
%		\includegraphics[width=3.2in]{fig/plt_timeseries_old_nc.png}
%		\caption{PLT timeseries -- Scenario 2}
%		\label{f:plt_timeseries_old_nc}
%%		\vspace{-0.2in}
%	\end{center}
%\vspace{-0.2in}
%\end{figure}



==> traffic_size.tex <==
%\subsubsection{Impact of traffic size}
\textbf{\sysname outperforms the baseline algorithms for any traffic size.}
%\obj{number of connections vs plt improvement plot}

Our design, explicitly addresses data sampling issue by introducing contextual bandits to help effectively guide the exploration through the configuration space.

In this section, we compare the impact of these contextual bandits by comparing \sysname with both bandits against a version of \sysname without the contextual bandits (i.e., DT) and a version with only \BO (BO).  In Figure~\ref{f:traffic-size}, we observe that with smaller number of connections (less than 10K), DT performs significantly worse than BO. However, with significantly more data, the two perform comparable and the DT still performs slightly worst than \sysname. Contextual bandits provides \sysname with a unique advantage which is crucial when samples are small, i.e., during bootstrapping and in tail conditions, but persists when samples are large. 

%In this section, we compare the impact of these contextual bandits by comparing \sysname with both bandits (\sysname-Bandits) against a version of \sysname without the contextual bandits (i.e., \sysname-DT) and a version with only \BO (\sysname-BO).  In Figure~\ref{f:traffic-size}, we observe that with smaller network classes (less than 10K), \sysname-DT performs significantly worse than \sysname-Bandits. However, with significantly more data, the two perform comparable and the \sysname-DT still performs slightly worst than \sysname-Bandits. Contextual bandits provides \sysname with a unique advantage which is crucial when samples are small, i.e., during bootstrapping and in tail conditions, but persists when samples are large. 

\label{s:traffic-size}

% \begin{figure}[tbh!]
%	\begin{center}
%		\includegraphics[width=3.4in]{fig/comp_fusion_box_comb.eps}
%		\caption{Impact of traffic size on learning}
%		\label{f:traffic-size}
%	\end{center}
%\end{figure}



% \begin{figure}[tbh!]
% 	\begin{center}
% 		\includegraphics[width=3in]{fig/median_comp_comb_logscale.png}
% 		\caption{Impact of traffic size on learning}
% 		\label{f:traffic-size}
% 	\end{center}
% \end{figure}
%
% \begin{figure}[tbh!]
%	\begin{center}
%		\includegraphics[width=3in]{fig/median_comp_comb_logscale_candle1.png}
%		\caption{Impact of traffic size on learning}
%		\label{f:traffic-size}
%	\end{center}
%\end{figure}

%  \begin{figure}[tbh!]
% 	\begin{center}
% 		\includegraphics[width=3in]{fig/decision_analysis_ml_ls.png}
% 		\caption{Decisions made using DT}
% 	\end{center}
% \end{figure}
%
%  \begin{figure}[tbh!]
% 	\begin{center}
% 		\includegraphics[width=3in]{fig/decision_analysis_sl_ls.png}
% 		\caption{Decisions made using BO}
% 	\end{center}
% \end{figure}

% \digdeep{What's the relation of learning algo with traffic size? Why SL works better initially? Why ML works better when traffic size rises? Why are there slight dips around 10000 region in SL?}
%
% \reword{
% Next, we modify our simulator to explore the effectiveness of learning algorithms as a function of number of connections. The simulations are run multiple times, with number of connections varied in each iteration. Figure \ref{f:traffic-size} plots the the median improvement in PLT for the two learning strategies, with number of connections varied from 1,000 to 1M. When the number of available data points is small, SL is able to make better decisions, as its exploration is guided by acquisition function. However, as the number of data points increases, ML performs better as it is able to generalize learning decisions across network classes. The dips is median improvement for \SL when traffic size is between 5000-10000 is attributed to connections from unseen network conditions that trigger creation of a new network class (and hence a new BO model from scratch). Whereas we do not observe similar dips for \ML due to its ability to jump-start the learning process for a new network class by using the trend seen in past.
% Moreover, SL's sensitivity to stopping criteria (EI) forces it improvements to cap at around 8\% for a certain network class. Although \sysname incorporates a \textit{Degree of Randomness} to keep exploration for better configurations going, its more effective for ML due to its ability to look across network classes. Once stopping criteria are met for SL, the model for a certain network class only gets updated when a better configuration is observed (due to random exploration) for a constituent of that \textbf{\textit{specific}} network class. Whereas for ML, a better configuration seen for a constituent of \textbf{\textit{any}} network class updates the model.
% }

==> web-complexity-eval.tex <==
\subsection{Impact of web complexity on learning}
\label{s:web-complexity-eval}
\obj{How does learning from one website translate tp another website? Do the optimal configurations remain the same?}

Websites can be radically divergent in their complexity (number and size of objects), with complex dependencies between the different resources \cite{}. It has already been observed that this complexity can impact performance of different HTTP versions \cite{}. We set out to understand the impact of web complexity on learning performance. Generalizing a set of website to a single trend can have benefits in terms of exploration and computing performance as a single BO model can fit a set of websites. In order to understand the impact of web complexity, we generalize the learning from website to its entire category. Instead of searching out for optimal configuration for each individual website, this flavor of \sysname picks one website as the basis of exploration/exploitation and generalizes the learning to its entire category. As a result, the best configuration found for the basis website so far is used for each website belonging to its category. We categorize the websites manually into \textit{Search, News, Entertainment} and \textit{Shopping} categories. 

Figure 14 plots the \% improvement in PLT when standard \sysname (per website learning) is compared to the modified \sysname (learning only for the basis website chosen randomly from its category). As it can be seen, there are tremendous benefits of learning for each, individual website. The optimal configuration does not remain the same for each individual website, even though they are in same category. The smallest improvement is seen for \textit{Search} websites, owing to their simple structure. The improvement is tremendous for the rest of three categories, as their optimal configuration vary widely.

\begin{figure}[tb!]
	\begin{center}
%		\includegraphics[width=3in]{fig/web-complexity-plt.eps}
\includegraphics[width=2.8in]{fig/web-complexity-plt-box.eps}
		\caption{Impact of WebComplexity}
		\label{f:web-complexity}
%		\vspace{-0.2in}
	\end{center}
\end{figure}
